Active Learning for Graph Neural Networks via Node Feature Propagation

Graph Neural Networks (GNNs) for prediction tasks like node classification or edge prediction have received increasing attention in recent machine learning from graphically structured data. However, a large quantity of labeled graphs is difficult to obtain, which significantly limits the true success of GNNs. Although active learning has been widely studied for addressing label-sparse issues with other data types like text, images, etc., how to make it effective over graphs is an open question for research. In this paper, we present an investigation on active learning with GNNs for node classification tasks. Specifically, we propose a new method, which uses node feature propagation followed by K-Medoids clustering of the nodes for instance selection in active learning. With a theoretical bound analysis we justify the design choice of our approach. In our experiments on four benchmark datasets, the proposed method outperforms other representative baseline methods consistently and significantly.

==> sections/approach.tex <==
\newcommand{\graph}{G}
\newcommand{\nodeset}{V}
\newcommand{\node}{v}
\newcommand{\feature}{x}
\newcommand{\labely}{y}
\newcommand{\featuremat}{X}
\newcommand{\labelvec}{Y}
\newcommand{\numclass}{C}
\newcommand{\featurespace}{\gX}
\newcommand{\labelspace}{\gY}
\newcommand{\numtrain}{n}\newcommand{\model}{\gM}
\newcommand{\selected}[1]{\mathbf{s}^{#1}}
\newcommand{\algo}{\gA}

\section{Preliminaries}



% \subsection{Problem Definition}

In this section, we describe a formal definition for the problem of graph-based active learning under the node classification setting and introduce a uniform set of notations for the rest of the paper. 
% Specifically, we are interested in a $C$ class classification problem, where the observations $(X, Y, G)$ denotes features drawn from compact space $\gX$, labels from space $\gY = \{1, \dots, C\}$ and the linkage information (graph) $G$. 
% Naturally, one can not assume the independence of nodes as their neighboring information does suggest certain degree of correlation. However, to cast the problem into a similar setting as the traditional classification problem, let us assume that there exists a prior (infinite) graph $G_0$ along with a probability space $P_0$ and vertex set $V_0$, so that the observation $G$ is an induced graph from $G_0$ via $P_0$ and each node can be viewed as i.i.d. samples of $V_0$.


We are given a large graph $\graph=(\nodeset,E)$, where each node $\node\in \nodeset$ is associated with a feature vector $\feature_\node \in \featurespace\subseteq \R^d$, and a label $\labely_\node \in \labelspace= \{1,2,...,\numclass\}$. Let $\nodeset=\{1,2,...,n\}$, we denote the input  features as a matrix $X\in \R^{\numtrain\times d}$, where each row represents a node, and the labels as a vector $\labelvec=(\labely_1,...,\labely_\numtrain)$.
We also consider a loss function
$l(\model | \graph, \featuremat, \labelvec)$ that computes the loss over the inputs $(\graph, \featuremat, \labelvec)$ for a model $\model$ that maps $\graph, \featuremat$ to a prediction vector $\hat{\labelvec} \in \labelspace^{\numtrain}$. Same as previous works on deep learning theory  \citep{allen2018convergence,du2018gradient}, we assume that $l$ is Lipschitz with constant $\lambda$ and bounded in $[-L,L]$.

Following previous works on GNN\citep{cai2017active,hamilton2017inductive}, we consider the inductive learning setting; i.e., a small part of $\labelvec$ is revealed to the algorithm, and we wish to minimize the loss on the whole graph $l(\model | \graph, \featuremat, \labelvec)$.
% $\graph\times \featurespace\rightarrow \labelspace$ (here we slightly abuse the notation to denote that $\graph$ is also an input to $\model$). 
Specifically, an active learning algorithm $\algo$ is initially given the graph $\graph$ and feature matrix $ \featuremat$. 
In step $t$ of operation, it selects a subset $\selected{t}\subseteq [\numtrain]=\{1,2,...,\numtrain \}$, 
and obtains $\labely_i$ for every $i\in \selected{t}$. 
We assume $\labely_i$ is drawn randomly according to a distribution $\mathbb{P}_{y|x_i}$ supported on $\labelspace$; we use $\eta_c(v)=\Pr[y=c|v]$ to denote the probability that $y=c$ given node $v$, and $\eta(v)=(\eta_1(v),...,\eta_C(v))^T$.
Then $\algo$ uses $\graph, \featuremat$ and $\labely_i$ for  $i\in \selected{0}\cup \selected{1}\cup \cdots\cup \selected{t}$ as the training set to train a model, using training algorithm $\model$. The trained model is denoted as $\model_{\algo_t}$. If $\model$ is the same for all active learning strategies, we can slightly abuse the notation $\algo_t= \model_{\algo_t}$ to emphasize the focus of active learning algorithms. A general goal of active learning is then to minimize the loss under a given budget $b$:
\begin{equation}
    \min_{\selected{0}\cup \cdots\cup \selected{t}} \E[l(\algo_t|\graph, \featuremat, \labelvec)] \label{eqn:target}
\end{equation}
where the randomness is over the random choices of $\labelvec$ and $\algo$.
%As $\model$ has multiple choices, 
We focus on $\model$ being the Graph Neural Networks and their variants elaborated in detail in the following part.

\subsection{Graph Neural Network Framework}
% \textbf{Graph Neural Network Framework}
% \yx{define S.}
Graph Neural Networks define a multi-layer feature propagation process similar to Multi-Layer Perceptrons (MLPs). Denote the $k$-th layer representation matrix of all nodes as $\featuremat^{(k)}$, and $\featuremat^{(0)}\in \R^{n\times d}$ are the input node features. Graph Neural Networks (GNNs) differ in their ways of defining the recursive function $f$ for the next-layer representation:
\begin{align}
	\featuremat^{(k+1)}&\leftarrow f(\featuremat^{(k)};G,\Theta_k),
\end{align}
where $\Theta_k$ is the parameter for the $k$-th layer. Naturally, the input $\featuremat$ satisfies $\featuremat^{(0)}=\featuremat$ by definition.
\textbf{Graph Convolution Network (GCN)}.
A GCN \citep{kipf2016semi} has a specific form of the function $f$ as:
\begin{align}
	\featuremat^{(k+1)}&\leftarrow \text{ReLU}(S\featuremat^{(k)}\Theta_k),
\end{align}
where ReLU is the element-wise rectified-linear unit activation function \citep{nair2010rectified}, $\Theta_k$ is the parameter matrix used for transforming the size of feature representations to a different dimension and $S$ is the normalized adjacency matrix. Specifically, $S$ is defined as:
\begin{align}
    S=(I+D)^{-\frac{1}{2}}(A+I)(I+D)^{-\frac{1}{2}},
\end{align} where $A$ is the original adjacency matrix associated with graph $G$ and $D$ is the diagonal degree matrix of $A$. Intuitively, this operation updates node embeddings by the aggregation of their neighbors. The added identity matrix $I$ (equivalent to adding self-loops to $G$) acts in a similar spirit to the residual links \citep{he2016deep} in MLPs that bypasses shallow-layer representations to deep layers. By applying this operation in a multi-layer fashion, a GCN encourages nodes that are locally related to share similar deep-layer embeddings and prediction results thereafter.

For the classification task, it is normal to stack a linear transformation along with a softmax function to the representation in the final layer, so that each class could have a prediction score. That is,
\begin{align}
    \hat{Y}&=\text{softmax}(\featuremat^{(K)}\Theta_K),
\end{align}
where $\text{softmax}(\vx)=\exp(\vx)/\sum_{c=1}^C \exp(x_c)$ which makes the prediction scores have unit sum of 1 for all classes, and $K$ is the total number of layers. We use the GCN structure as the fixed unified model $\model$ for all the following discussed AL strategies $\algo$.% \yw{}
% \yw{note that data points are no-longer independent as the normalized adjacency matrix mingles their feature representations.}


% the GCN model, and each class-specific conditional probability $\eta_c(\vx)=p(y=c|\vx)$ to be $\lambda^\eta$-Lipschitz continuous for all $c$.


\section{Active Learning Strategy \& Theoretical Analysis}
% \begin{algorithm}[ht]
% 	\caption{Propagated Embedding Selection}
% 	\label{algo:K-Medoids}
% 	\begin{algorithmic}[1]        
% 		\Require{Representation matrix $\featuremat$, normalized adjacency matrix $S$ and a budget $b$}
% 		\State Compute propagated embeddings as $\featuremat'=S^k \featuremat$ \Comment{$k$ is the number of layers in the GCN}
% 		\State Perform K-Medoids over $\featuremat'$ with $b$ centers
% 		\State Select $\selected{}$ to be nodes that are closest to these centers\\
% 		\Return{$\selected{}$}
% 	\end{algorithmic}
% \end{algorithm}


% \yy{I rewrote this paragraph:}
%Traditionally, active learning choose labels in a purely sequential fashion, i.e., each time $\algo$ only queries one label, 
Traditionally, active learning algorithms choose one instance at a time for labeling, i.e.,
with $|\selected{t}|=1$. 
% However, such behavior is infeasible in practice mainly because of two reasons: i) Modern datasets contain very large numbers of points and it can be extremely time-consuming if we collect the labels one by one; ii) It is also infeasible to retrain the network at each step during the training process since it takes a long time. 
However, for modern datasets where the numbers of training instances are very large, it would be extremely costly if we re-train the entire system each time when a new label is obtained.
Hence we focus on the %\textit{one-step} 
% \yy{\textit{mini-batch}}
``batched'' one-step active learning setting \citep{contardo2017meta}, and select the informative nodes once and for all when the algorithm starts.
This is also called the \textit{optimal experimental design} in the literature \citep{Expdesign_book,DBLP:journals/corr/abs-1711-05174}. 
Aiming to select the $b$ most representative nodes as the batch, our target (\ref{eqn:target}) becomes:
\begin{equation}
    \min_{|\selected{0}|\leq b} \E[l(\algo_0|\graph, \featuremat, \labelvec)]. 
\end{equation}
%that aims at selecting 
% Our algorithm therefore focuses on the best method to select 
%the most representative points in $\nodeset$. 
% \yy{I rewrote the next paragraph, too:}
The node selection algorithm is described in Section~\ref{sec:pes}, followed by the loss bound analysis in Section~\ref{sec:pes_analysis}, and the comparison with a closely related algorithm (K-Center in Coreset \citep{sener2017active}) in Section~\ref{sec:not_coreset}. 
%In Section~\ref{sec:pes},  we give our \yw{Node Feature Propagation Selection} strategy, and present its theoretical analysis in Section~\ref{sec:pes_analysis}. Then, we give a comparison with the previous Coreset method in Section~\ref{sec:not_coreset}.


% \subsection{Propagated Embedding Selection with K-Medoids Clustering
\definecolor{my_blue}{rgb}{0.223, 0.770, 0.730}
% \definecolor{my_blue}{HTML}{7e80fc}

\subsection{Node Selection via Feature Propagation and K-Medoids Clustering%\yw{revisit this name in the context}
}
\label{sec:pes}
\begin{algorithm}[ht]
	\caption{Active Learning with Distance-based Clustering}
	\label{algo:K-Medoids}
	\begin{algorithmic}[1]        
		\Require{Node representation matrix $\featuremat$, graph structure matrix $G$ and budget $b$}
		\State Compute a distance function $d_{\featuremat, \graph}(\cdot,\cdot): \nodeset\times \nodeset \rightarrow \R $\label{alg:line:dist} \hfill \textcolor{my_blue}{\# for FeatProp: use Eqn. (\ref{eqn:dist})} %\yw{clearer notation}
% 		\State Compute propagated embeddings as $\featuremat'=S^k \featuremat$ \Comment{$k$ is the number of layers in the GCN}
% 		\State Perform K-Medoids over $d_{X,G}$ with $b$ centers\label{alg:line:kmean}
		\State Perform clustering using $d_{X,G}$ with $b$ centers\label{alg:line:kmean} \hfill \textcolor{my_blue}{\# for FeatProp: use K-Medoids}
		\State Select $\selected{}$ to be the centers
		\State Obtain labels for $v\in \selected{}$ and train model $\model$
		\Ensure{Model $\model$}
		\end{algorithmic}
\end{algorithm}

% \yy{Yuexin: Please re-order the paragraphs below: first, introduce the distance matrix, and then applies K-Medoids to the matrix and selects the $b=k$ centroids.}

% Our algorithm (Algorithm \ref{algo:K-Medoids}) acts in two steps: 
We describe a generic active learning framework using distance-based clustering in Algorithm \ref{algo:K-Medoids}. It acts in two major steps:
1) computing a distance matrix or function $d_{X,G}$ using the node feature representations $X$ and the graph structure $G$; 2) applying clustering with $b$ centers over this distance matrix, and from each cluster select the node closest to the center of the cluster. 
After receiving the labels (given by matrix $Y$) of the selected nodes, we train a graph neural network, specifically GCN, based on $X, G$ and $Y$ for the node classification task.  
% The procedure is described in detail in Algorithm~\ref{algo:K-Medoids}. 
Generally speaking, different options for the two steps above would yield different performance in the down-stream prediction tasks; we detail and justify our choices below and in subsequent sections.
% which we will analyze theoretically in Section~\ref{sec:not_coreset} and examine empirically in Section~\ref{sec:exp_res}.

% Here, we discuss a \yw{direct} yet effective design choice for these consecutive procedures.

% We consider a simple K-Medoids based active learning algorithm, presented in Algorithm \ref{algo:K-Medoids}; we first compute a distance matrix $d_{X,G}$ based on the input, and run $k$-MedoidK-Meanrithm on the distance matrix to select $b$ centers. 

%Note that the distance is fully defined by the input feature $X$ and the graph structure $G$, and early trials in the general active learning setting
\textbf{Distance Function.} Previous methods \citep{sener2017active,cai2017active,gao2018active} commonly use network representations to compute the distance, i.e., $d_{X,G}(v_i,v_j)=\|(X^{(k)})_i- (X^{(k)})_j\|_2$ for some specific $k$. While this can be helpful in a well-trained network, the representations are quite inaccurate in initial stages of training and such distance function might not select the representatitive nodes.
% Note that our distance matrix depends on both the node features in $X$ and the graph structure in $G$, while traditional active learning strategies only use $X$ but do not take $G$ into consideration \citep{DBLP:journals/jmlr/BodoMC11,sener2017active}.
%For example, %It only remains to specify the distance matrix $d_{X,G}$. 
%previous methods suggest using L2 distance\citep{sener2017active} or kernel methods \citep{DBLP:journals/jmlr/BodoMC11} over $X$ alone. % These methods cannot take $G$ into account. 
% \yy{I reworded the next}:
%Here, we adopt a direct yet effective design choice for these consecutive procedures. That is, 
Differently, we define the pairwise node distance using the $L_2$ norm of the difference between the corresponding
%for distance $d_{G,X}$ we propose to use L2 over the 
propagated node features: 
\begin{align}
    d_{X,G}(v_i,v_j)=\|(S^KX)_i- (S^KX)_j\|_2, \label{eqn:dist}
\end{align} 
% \textcolor{red}{AS: is this $S^K$ same as $S^k$? Otherwise define what K means.}
where $(M)_i$ denotes the $i$-th row of matrix $M$, and recall that $K$ is the total number of layers. Intuitively, this removes the effect of untrained parameters on the distance, while still taking the graph structure into account.
% \yx{I changed the order of these sentences}
%And for the clustering sub-routine, 
% Intuitively, the propagated features in our approach act as the surrogates of the GCN hidden representations. 

\textbf{Clustering Method.} Two commonly used methods are K-Means \citep{cai2017active,gao2018active} and K-Center \citep{sener2017active}\footnote{For a group of nodes, K-Center problem aims to find a $\delta$-cover with at most $k$ nodes for smallest possible $\delta$.}. We propose to apply the K-Medoids clustering. K-Medoids problem is similar to K-Means, but the center it selects must be real sample nodes from the dataset. This is critical for active learning, since we cannot try to label the unreal cluster centers produced by K-Means.
Also, we show in Section \ref{sec:not_coreset} that K-Medoids can obtain a more favorable loss bound than K-Center.
% to the distance matrix, where each row is treated as the vector representation of each node. % \yy{I rewrote the next paragraph;}
%We call our algorithm Propagated Embedding Selection (PES) as $S^kX$ reflects the propagation characteristics of the input features between locally-connected nodes.
%Notably, % each used option has its own reason 
%\yw{each option is chosen based on its intuitive yet provable characteristics}. Roughly speaking, 
% The K-Medoids clustering
%can be proved to derive a 
% yields a tighter loss bound than K-Center, the clustering method employed by \cite{sener2017active}, as we justify theoretically in the next two sections. 
% After receiving the labels (given by matrix $Y$) of the selected nodes, we train a graph neural network, specifically GCN, based on $X, G$ and $Y$ for the node classification task.  

We call our method \textit{FeatProp}, to emphasize the active learning strategy via node feature propagation over the input graph, which is the major difference from other node selection methods. 
% We specify our choices for distance function and clustering method i
% (Section~\ref{sec:exp_res}).


\subsection{Theoretical Analysis of Classification Loss Bound}
\label{sec:pes_analysis}

\newcommand{\gtmodel}{\model^*}
\newcommand{\almodel}{\algo_0}
\newcommand{\modelpred}[2]{(#1)_{#2}}
\newcommand{\lip}{\lambda}
\newcommand{\lossbound}{L}
%In this section we give theoretical justification on using L2 over propagated embedding as distance function. Basically, we use 
Recall that we use $\|(S^KX)_i- (S^KX)_j\|_2$ to approximate the pairwise distances between the hidden representations of nodes in GCN.   
% \yy{I am not sure your statement here is convincing so I delete it.}
%This means that we can obtain a small classification error for the trained GCN if the error for these surrogate representations is also small \yw{rephrase}. 
Intuitively, representation $S^KX$ resembles the output of a simplified GCN  \citep{wu2019simplifying} by dropping all activation functions and layer-related parameters in the original structure, which introduces a strong inductive bias.
% (thus with small variance due to bias-variance tradeoff). 
In other words, the selected nodes could possibly contribute to the stabilization of model parameters during the training phase of GCN. The following theorem formally shows that using K-Medoids with propagated features can lead to a low classification loss:
\begin{theorem}[informal]
\label{th:main}
Suppose that the label vector $Y$ is sampled independently from the distribution $y_i\sim \eta(i)$, and the loss function $l$ is bounded by $[-\lossbound,\lossbound]$. Then under mild assumptions, there exists a constant $c_0$ such that with probability $1-\delta$ the expected classification loss of $\algo_t$ satisfies
\begin{equation}
\begin{aligned}
    \frac{1}{n}l(\algo_0|\graph,\featuremat,\labelvec)\leq& \frac{c_0}{n}\sum_{i=1}^n \min_{j\in \selected{0}}\|(S^KX)_i-(S^KX)_j\|_2 \\&+ \sqrt{\frac{\lossbound\log(1/\delta)}{2n}} \label{eqn:bound_kmeans}
\end{aligned}
\end{equation}
\end{theorem}
To understand Theorem \ref{th:main}, notice that the first term $\sum_{i=1}^n \min_{j\in \selected{0}}\|(S^KX)_i-(S^KX)_j\|_2$ is exactly the target loss of K-Medoids (sum of point-center distances), and the second term $\sqrt{\frac{\lossbound\log(1/\delta)}{2n}}$ quickly decays with $n$, where $n$ is the total number of nodes in graph $G$. Therefore the classification loss of $\almodel$ on the entire graph $G$ is mostly dependent on the K-Medoids loss. In practice, we can utilize existing robust initialization algorithms such as Partitioning Around Medoids (PAM) to 
%\yx{\sout{boost the performance.} 
approximate the optimal solution for K-Medoids clustering.

% \begin{wrapfigure}{r}{0.4\textwidth}
% % \begin{wrapfigure}{r}{0pt}
%   \begin{center}
%     \includegraphics[width=0.4\textwidth]{vis.pdf}
%   \end{center}
%   \caption{Visualization of Theorem~\ref{th:main}. Consider the set of selected points \textcolor{blue}{$\selected{}$} and the remaining points in the dataset \textcolor{red}{$[\numtrain]\backslash \selected{}$}. It suggests from our theorem that the K-Medoids paradigm gives a bound of $\gO(\sum_i d_i/n)+\gO(\sqrt{\frac{1}{n}})$ while K-Center (Section~\ref{sec:not_coreset}) shows $\gO(\max_i d_i)+\gO(\sqrt{\frac{1}{n}})$, which is looser than the former one.}
%     \label{fig:vis}
% \end{wrapfigure}


The assumptions we made in Theorem \ref{th:main} are pretty standard in the literature. For the integrity of the paper, we defer the proof details to Section \ref{sec:proofs}. While our results share some common characteristics with Sener et al.\citep{sener2017active}, our proof is more involved in the sense that it relates to the translated features $\|(S^KX)_i-(S^KX)_j\|_2$ instead of the raw features $\|(X)_i-(X)_j\|_2$. In fact, we conjecture that using raw feature clustering selection for GCN will not result in a similar bound as in (\ref{eqn:bound_kmeans}): this is because GCN uses the matrix $S$ to diffuse the raw features across all nodes in $\nodeset$, and the final predictions of node $i$ will also depend on its neighbors as well as the raw feature $(X)_i$.
% Note that relating the loss to propagated features rather than raw features is desirable, as the latter one without the consideration of graph structures will usually result in a worse performance.
% In fact, using raw feature clustering instead of the propagated features will not result in a bounded classification loss for GCN, because GCN uses the matrix $S$ to diffuse the features across all nodes in $\nodeset$. 
We could see a clearer comparison in practice in Section~\ref{sec:exp_res}.
% \yw{Intuitively, this suggests that we minimize over the summation of point-center distances.}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.8\linewidth]{vis.pdf}
    \caption{Visualization of Theorem~\ref{th:main}. Consider the set of selected points \textcolor{blue}{$\selected{}$} and the remaining points in the dataset \textcolor{red}{$[\numtrain]\backslash \selected{}$}. 
    K-Medoids corresponds to the mean of all red segments in the figure, whereas K-Center corresponds to the max of all red segments in the figure.
%    	It suggests from our theorem that the K-Medoids paradigm gives a bound of $\gO(\sum_i d_i/n)+\gO(\sqrt{\frac{1}{n}})$ while K-Center (Section~\ref{sec:not_coreset}) shows $\gO(\max_i d_i)+\gO(\sqrt{\frac{1}{n}})$, which is looser than the former one.
    }
    \label{fig:vis}
\end{figure}

\newcommand{\coversize}{d}
\subsection{Why not K-Center}
\label{sec:not_coreset}
In this subsection we provide justifications on using the K-Medoids clustering method as opposed to Coreset \citep{sener2017active}. The Coreset approach aims to find a $\delta$-cover of the training set. In the context of using propagated features, this means solving
\begin{equation}
\begin{aligned}
\delta&=\min_{|\selected{0}|\leq b}\max_i \min_{j\in \selected{0}} d_{\featuremat, \graph}(\node_i, \node_j)\\& =  \min_{|\selected{0}|\leq b}\max_i \min_{j\in \selected{0}} \|(S^KX)_i-(S^KX)_j\|_2 \label{eqn:bound_cover}
\end{aligned}
\end{equation}


We can show a similar theorem as Theorem \ref{th:main} for the Coreset approach:
\begin{theorem}\label{thm:bound_center}
	Under the same assumptions as in Theorem \ref{th:main}, with probability $1-\delta$ the expected classification loss of $\algo_t$ satisfies 
	 \begin{equation}
	 \begin{aligned}
	     \frac{1}{n}l(\algo_0|\graph,\featuremat,\labelvec)\leq &c_0\max_i \min_{j\in \selected{0}} \|(S^KX)_i-(S^KX)_j\|_2 \\&+ \sqrt{\frac{\lossbound\log(1/\delta)}{2n}}
	%  \frac{1}{n}\sum_{i=1}^n \min_{j\in \selected{0}}\|(S^KX)_i-(S^KX)_j\|_2\leq \. 
	 \end{aligned}
	\end{equation}
\end{theorem}

Let $d_i = \min_{j\in \selected{0}} \|(S^KX)_i-(S^KX)_j\|_2$. It is easy to see that RHS of Eqn. (\ref{eqn:bound_kmeans}) is smaller than RHS of Eqn. (\ref{eqn:bound_cover}), since $\frac{1}{n}\sum_{i=1}^n d_i\leq \max_i d_i$. In other words, K-Medoids can obtain a better bound than the K-Center method (see Figure \ref{fig:vis} for a graphical illustration). We observe superior performance of K-Medoid clustering over K-Center clustering in our experiments as well (see Section \ref{sec:exp_res}).

% In fact, our method can also apply to the standard neural networks analyzed in \citep{sener2017active}, and it is interesting to analyze the effect of replacing K-Center with K-Medoids for image classification tasks in the future work.

%Besides the propagated features used to compute centers, another important factor of our algorithm is the K-Medoids clustering. The most related work to our center finding procedure is the K-Center approach in Coreset \citep{sener2017active}, that tries to minimize
%  as opposed to the K-Center option: minimizing 
% the largest point-center distance: 
% \begin{align}
% \min_{|\selected{0}|\leq b}\max_i \min_{j\in \selected{0}} d_{\featuremat, \graph}(\node_i, \node_j)    
% \end{align}
% where the distance function is defined by the dot-product operation between feature representations in the final layer $\featuremat^{(K)}$. For the final clustering method (Line~\ref{alg:line:kmean} in Algorithm~\ref{algo:K-Medoids}), we choose to use K-Medoids instead of $k$K-Centr mainly due to two reasons: \\
% 1) Under similar assumptions as in Theorem~\ref{th:main}, we could see that K-Center is confined to a looser bound in terms of the total loss; that is:
% \begin{equation}
%\frac{1}{n}l(\algo_t|\graph,\featuremat,\labelvec)\leq c_0\max_i \min_{j\in \selected{0}} \|(S^KX)_i-(S^KX)_j\|_2 + \sqrt{\frac{\lossbound\log(1/\delta)}{2n}}
%  \frac{1}{n}\sum_{i=1}^n \min_{j\in \selected{0}}\|(S^KX)_i-(S^KX)_j\|_2\leq \. 
%\end{equation}

% \begin{theorem}
% \label{th:kcenter}
% Suppose the set $\selected{0}$ is a $\coversize$-cover of the nodes under the distance defined by $S^KX$, i.e.,  $\max_{i\in \nodeset}\min_{j\in \selected{0}}\|(S^KX)_i-(S^KX)_j\|_2\leq \delta$.
% Under the same assumptions and the same constant $c_0$ as in Theorem \ref{th:main}, with probability $1-\delta$ the expected inductive loss of $\algo_t$ satisfies
% \begin{equation}
%   \frac{1}{n}l(\algo_t|\graph,\featuremat,\labelvec)\leq c_0\coversize + \sqrt{\frac{\lossbound\log(1/\delta)}{2n}}   \label{eqn:bound_coreset}
% \end{equation}
% \end{theorem}
% The first term, proportional to the maximum of point-center distance, is larger than the mean point-center distance counter-part in K-Medoids. We visualize the difference in Figure~\ref{fig:vis}. \\
% 2) As K-Center is NP-Hard \citep{har2011geometric}, in order to get a more accurate solution, people use mixed integer programming (MIP) \citep{sener2017active} as the approximated algorithm, which can be much more time-consuming than K-Medoids based on Expectation Maximization (EM). An alternative solution is to use a greedy selection paradigm specified in Algorithm~\ref{algo:$k$-Cknter}. While being more efficient, the greedy algorithm will have inferior performances to MIP in applications such as image classifications with CNNs \citep{sener2017active}. We will elaborate more on these points in the Section~\ref{sec:exp_res}.

% \yw{pictures showing the difference of K-Medoids and K-Center}

% \yw{may delete the algorithm, its only a greedy-approximation}


%\begin{algorithm}[ht]
%	\caption{K-Center-Greedy%\yw{modify for }
%	}
%	\label{algo:$k$-Ck-center}
%	\begin{algorithmic}[1]        
%		\Require{Distance function $d_{\featuremat, \graph}(\cdot,\cdot)$, % $\featuremat^{(K)}$, 
%		existing pool $\selected{0}$ and a budget $b$}
%		\State Initialize $\selected{}=\selected{0}$\Comment{Warm start, $\selected{0}$ can be a small random selection}
%		\Repeat
%% 		\State $u=\arg\max_{i\in [\numtrain]\backslash \selected{}}\min_{j\in\selected{}}\Delta((\featuremat)^{(K)}_i,(\featuremat)^{(K)}_j)$
%		\State $u=\arg\max_{i\in [\numtrain]\backslash \selected{}}\min_{j\in\selected{}}d_{\featuremat, \graph}(\node_i,\node_j)$
%		\State $\selected{}=\selected{}\cup \{u\}$ 
%		\Until{$|\selected{}|=b+|\selected{0}|$}\\
%		\Return{$\selected{}$}
%	\end{algorithmic}
%\end{algorithm}

% \yw{tighter bound, illustrated in the experiment section}

% \yw{computation time, so in reality, people use $k$K-Center illustrated in the experiment section}



==> sections/conclusion.tex <==
\section{Conclusion}
We study the active learning problem in the node classification task for Graph Convolution Networks (GCNs). We propose a propagated node feature selection approach (FeatProp) to comply with the specific structure of GCNs and give a theoretical result characterizing the relation between its classification loss and the geometry of the propagated node features. Our empirical experiments also show that FeatProp outperforms the state-of-the-art AL methods consistently on most benchmark datasets. Note that FeatProp only focuses on sampling representative points in a meaningful (graph) representation, while uncertainty-based methods select the active nodes from a different criterion guided by labels, how to combine that category of methods with FeatProp in a principled way remains an open and yet interesting problem for us to explore.

==> sections/exp.tex <==
\section{Experiment}
%\subsection{Synthesized Experiment}
% \subsection{Experiment Details}

% \subsection{Dataset}
We evaluate the node classification performance of our selection method on the Cora, Citeseer, and PubMed network datasets \citep{yang2016revisiting}. We further supplement our experiment with an even denser network dataset CoraFull \citep{bojchevski2017deep} to illustrate the performance differences of the comparing approaches on a large-scale setting. Table~\ref{tab:dataset} summarizes the dataset statistics.

\begin{table}[ht]
    \centering
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{c|cccc}
        \toprule
        Data &\# Nodes &\# Edges &\# Classes & Feature size\\
        \midrule
        Cora & 2,708 &5,429 & 7 &3,703\\
        Citeseer & 3,327 &4,732 & 6 &1,433\\
        PubMed &19,717 &44,338 & 3 &500\\
       CoraFull &19,793 &126,842 &70 &8,710\\
        \bottomrule
    \end{tabular}%
    }
    \caption{Dataset statistics of different networks.}
    \label{tab:dataset}
\end{table}%


\begin{table}[ht]
    \centering
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{c|cccc}
        \toprule
         & Cora & Citeseer &PubMed &CoraFull \\
        \midrule
        FeatProp & 239 & 622 & 1,506 &13,059\\
        CoresetMIP & 12,260 &13,257 & OOT &OOT\\
        Coreset-greedy & 44 & 46 & 509 & 636\\
        \bottomrule
    \end{tabular}%
    }
    \caption{Comparison of running time of 5 different runs in seconds between our algorithm (FeatProp) and Coreset. OOT denotes out-of-time. Note in order to get a more accurate solution, CoresetMIP costs much more time than Coreset-greedy.}
    \label{tab:time}
\end{table}

\begin{table*}[ht] \centering \begin{tabular}{c|cccc} \toprule
 &Cora &Citeseer &PubMed &CoraFull\\
\midrule
Random &$59.83 \pm5.77$ &$48.79 \pm4.03$ &$71.66 \pm4.50$ &$10.75 \pm0.92$\\
Degree &$63.30 \pm0.55$ &$35.50 \pm0.82$ &$60.54 \pm0.38$ &$10.85 \pm0.30$\\
Uncertainty &$48.14 \pm8.18$ &$39.14 \pm4.52$ &$64.80 \pm8.21$ &$6.76 \pm0.72$\\
Coreset-greedy &$59.99 \pm4.59$ &$48.21 \pm3.78$ &$68.41 \pm4.50$ &$10.83 \pm1.28$\\
CoresetMIP &$55.86 \pm6.89$ &$46.76 \pm3.99$ &$-$ &$-$\\
AGE &$65.01 \pm2.43$ &$49.65 \pm5.19$ &$67.96 \pm2.73$ &$13.52 \pm0.81$\\
ANRMAB &$63.71 \pm4.34$ &$47.29 \pm3.33$ &$71.06 \pm4.82$ &$11.40 \pm0.98$\\
FeatProp &$\bm{74.89 \pm2.63}$ &$\bm{51.03 \pm2.80}$ &$\bm{73.20 \pm1.81}$ &$\bm{14.86 \pm0.70}$\\
\bottomrule \end{tabular} 
\caption{Comparison of Macro-F1$\pm$standard\_deviation averaged over different number of labeled nodes for training. Bold fonts represent the best methods. CorsetMIP does not scale up for PubMed and CoraFull datasets.}
\label{tab:macro-f1-gcn}
\end{table*}

We evaluate the % \yx{inductive} 
Macro-F1 of the methods over the full set of nodes. The sizes of the budgets are fixed for all benchmark datasets. Specifically, we choose to select $10, 20, 40, 80$ and $160$ nodes as the budget sizes. After selecting the nodes, a two-layer GCN \footnote{In the past semi-supervised setting of citation networks, a two-layer GCN is the optimal structure for the node classification task \citep{kipf2016semi}. %the performances of GCNs are not sensitive to the number of layers. We choose this layer number as the result of both performance and efficiency considerations.
}, with $16$ hidden neurons, is trained as the prediction model. We use the Adam \citep{kingma2014adam} optimizer with a learning rate of $0.01$ and weight decay of $5\times 10^{-4}$. All the other hyperparameters are kept as in the default setting ($\beta_1=0.9,\beta_2=0.999$). To guarantee the convergence of the GCN, the model trained after $200$ epochs is used to evaluate the metric on the whole set. %\footnote{Note in this graph AL setting, we do not have a validation set.} %\yx{Is the best performance over 200 epochs chosen, or we evaluate at exactly 200 epochs?}
\subsection{Baselines}
\label{exp:comparing_methods}
We compared the following methods:
% We compared our AL strategy (FeatProp) with other representative strategies listed below: %\yx{I changed the wording a little bit}
% \yw{all the strategies share the same GCN structure after the selection of nodes}
\begin{itemize}
    % \item \yw{Baseline explanation}
    \item \textbf{Random:} Choosing the nodes uniformly from the whole vertex set.
    \item \textbf{Degree:} Choosing the nodes with the largest degrees. Note that this method does not consider the information of node features.
    % \item \textbf{FeatureClustering:} This method performs a K-Means clustering over the raw features. Nodes that have the closest representations to the centers are selected. This method does not consider the graph structure.
    \item \textbf{Uncertainty:} Similar to the methods in \cite{joshi2009multi}, we put the nodes with max-entropy % and max-margin (i.e. difference between best and second-best scores) 
    into the pool of instances. % \yw{whether to use a more accurate term.}
    \item \textbf{Coreset \citep{sener2017active}:} This method performs a K-Center clustering over the last hidden representations in the network. If time allows (on Cora and Citeseer), a robust mixture integer programming method as in \cite{sener2017active} (dubbed CoresetMIP) is adopted. We also apply a time-efficient approximation version (Coreset-greedy) % see Algorithm~\ref{algo:k-center}) 
    for all of the datasets. The center nodes are then selected into the pool. % In our experiments, we observe no explicit difference between CoresetMIP and Coreset-greedy.
    \item \textbf{AGE \citep{cai2017active}:} This method linearly combines three metrics -- graph centrality, information density, and uncertainty and select nodes with the highest scores.
    \item \textbf{ANRMAB \citep{gao2018active}:} This method enhances AGE by learning the combination weights of metrics through an exponential multi-arm-bandit updating rule.
    \item \textbf{FeatProp:} This is our method. We perform a K-Medoids clustering to the propogated features (Eqn. (\ref{eqn:dist})), where $X$ is the input node features. In the experiment, we adopts an efficient approximated K-Medoids algorithm which performs K-Means until convergence and select nodes cloesest to centers into the pool. 
    % Note that the distance function in our algorithm is based on (\ref{eqn:dist})
\end{itemize}

%\begin{figure}[htb]
%    \centering
%    \begin{subfigure}[b]{\textwidth}
%        \centering
%        \includegraphics[width=0.475\linewidth]{Cora.pdf}%
%        \hfill
%        \includegraphics[width=0.475\linewidth]{Citeseer.pdf}%
%    \end{subfigure}
%    \vskip\baselineskip
%    \begin{subfigure}[b]{\textwidth}
%        \centering
%        \includegraphics[width=0.475\linewidth]{PubMed.pdf}%
%        \hfill
%        \includegraphics[width=0.475\linewidth]{CoraFull.pdf}%
%    \end{subfigure}
%    \caption{Results of different approaches over benchmark datasets ( averaged from 5 different runs).}
%    \label{fig:main}
%\end{figure}

\begin{figure*}[htb]
    \centering
    \includegraphics[width=0.82\linewidth]{figs_uai/All_macro.pdf}%
    \caption{Results of different approaches over benchmark datasets averaged from 5 different runs.}
\label{fig:main}
\end{figure*}

\subsection{Experiment Results}
\label{sec:exp_res}
% We conducted experiments on active learning for all approaches. 
In our experiments, we start with a small set of nodes (5 nodes) sampled uniformly at random from the dataset as the initial pool. We run all experiments with 5 different random seeds and report the averaged classification accuracy as the metric. We plot the accuracy vs the number of labeled points. For approaches (Uncertainty, Coreset, AGE and ANRMAB) that require the current status/hidden representations from the classification model, a fully-trained model built from the previous budget pool is returned. For example, if the current budget is $40$, the model trained from $20$ examples selected by the same AL method is used. %\yw{We run the query algorithm iteratively; in other words, we solve the discrete optimization problem}

\textbf{Main results.} % \yw{update analysis with new baselines} 
As is shown in Figure~\ref{fig:main}, our method outperforms all the other baseline methods in most of the compared settings. It is noticeable that AGE and ANRMAB which use uncertainty score as their sub-component can achieve better performances than Uncertainty and are the second best methods in most of the cases. 
% Note that Coreset and Uncertainty focus on exactly different selection criteria -- either expressiveness of features or the current model confidence. We believe that the observation there is no clear clue for which method is superior is partially due to the fact that datasets of different characteristics favor distinct selection aspects.  % Furthermore, note that FeatureClustering cannot achieve even close performances as FeatProp in most of the datasets, which suggests that the raw features alone have quite different geometry distribution as the propagated ones. 
% It is noticeable that Random could achieve relatively good performances on small datasets (Cora and Citeseer). When the vertex size (PubMed and CoraFull) grows, which may require more insightful guidance from graphs and features, Random will no longer give out good scores. \yw{previous sentence not reliable}
% Moreover, it is interesting to find that in CoraFull with the densest linkage structure, Degree, which utilizes the graph information alone could produce a good result and is even better than other active learning baselines.  We believe that this is due to the fact that methods (Uncertainty/Coreset) requiring model statuses/hidden representations can be highly-unstable and are more likely to sample biased nodes with an overfitted model resulting from the small number of training points.
% the vast number of % as CoraFull has a total of $70$ different 
% classes, which is larger than most of the sample budgets.\yx{I feel it better not to emphasize \#nodes<\#classes here - this is kind of weird. Let's discuss}
% In this case, strong guidance from the graph structure helps more. Naturally, FeatProp with no dependence on GCN parameters will also be stable. 
We also show an averaged Macro-F1 with standard deviation across different number of labeled nodes in Table~\ref{tab:macro-f1-gcn}. It is interesting to find that our method has the second smallest standard deviation (Degree is deterministic in terms of node selection and the variance only comes from the training process) among all methods. We conjecture that this is due to the fact that other methods building upon uncertainty may suffer from highly variant model parameters at the beginning phase with very limited labeled nodes.

%\yw{noticeable that methods that neglect information such as Degree FeatureClustering usually have the worst performance among all methods} 

\textbf{Efficiency.} % \yw{comparison of time} 
We also compare the time expenses between our method and Coreset, which also involves a clustering sub-routine (K-Center), %Algorithm \ref{algo:k-center}) 
in Table~\ref{tab:time}. It is noticeable that in order to make Coreset more stable, CoresetMIP uses an extreme excess of time comparing to Coreset-greedy in the same setting.
% the extra large amount of time cost for the CoresetMIP version is unavoidable \yx{does unavoidable mean large here?} while the greedy algorithm takes much less time on the same setting. 
An interesting fact we could observe in Figure~\ref{fig:main} is that CoresetMIP and Coreset-greedy do not have too much performance difference on Citeseer, and Coreset-greedy is even better than CoresetMIP on Cora. This is quite different from the result in image classification tasks with CNNs \citep{sener2017active}. This phenomenon distinguishes the difference between graph node classification with traditional classification problems. We conjecture that this is partially due to the fact that the nodes no longer preserve independent embeddings after the GCN structure, which makes the original analysis of Coreset not applicable. %\yw{whehther this analysis is valid}

\begin{figure*}[htb]
    \centering
    % \includegraphics[width=0.85\linewidth]{kcenter_kmeans.pdf}%
    \includegraphics[width=0.85\linewidth]{kcenter_kmeans_macro.pdf}%
    \caption{Results of different approaches over benchmark datasets averaged from 5 different runs. Similar to Coreset, the orange line denotes replacing the original distance function in Eqn. (\ref{eqn:dist}) with L2 distance from the final GCN layer. The blue line denotes the algorithm replacing the K-Medoids module with K-Center clustering.
    }
    \label{fig:kcenter_kmeans}
\end{figure*}

%\begin{figure}[htb]
%    \centering
%    \includegraphics[width=0.85\linewidth]{kcenter_kmeans_kl.pdf}%
%    \caption{KL Divergence of the label of selected nodes vs true label distribution of different approaches over benchmark datasets aggregated from 5 different runs. FeatProp-kcenter denotes the algorithm replacing the K-Means module with K-Center clustering. The lower, the better.}
%    \label{fig:kcenter_kmeans_kl}
%\end{figure}
% \textbf{K-Center replacement.}
\textbf{Ablation study.}
It is crucial to select the proper distance function and clustering subroutine for FeatProp (Line~\ref{alg:line:dist} and Line~\ref{alg:line:kmean} in Algorithm~\ref{algo:K-Medoids}). As is discussed in Section~\ref{sec:not_coreset}, we test the differences with the variant of using the L2 distance from the final layer of GCN as the distance function and the one by setting K-Medoids choice with a K-Center replacement.
%It is possible to replace the K-Means clustering module in Algorithm ~\ref{algo:k-means} with the counter-part in Coreset (K-Center).
We compare these algorithms in Figure~\ref{fig:kcenter_kmeans}. As is demonstrated in the figure, the K-Center version (blue line) has a lower accuracy than the original FeatProp approach. This observation is compatible with our analysis in Section~\ref{sec:not_coreset} as K-Medoids comes with a tighter bound than K-Center in terms of the classification loss. Furthermore, as final layer representations are very sensitive to the small budget case, we observe that the network representation version (orange line) also generally shows a much deteriorated performance at the beginning stage. % We further investigate the sampled label distributions from these two methods and compute their KL-divergence with respect to the true label distribution in Figure~\ref{fig:kcenter_kmeans_kl}. We can perceive that FeatProp retrieves a more real-data-like sample set while FeatProp-kcenter is more biased, which we conjecture \yw{wording} is the main cause of its inferior performance.
%\yw{replace the clustering method with K-Center}

% \yw{comparison of label distribution, seems like that the distribution is not the closest to the true label distribution}
% \yw{here only put the comparison of label distributions related to FeatProp and FeatProp-kcenter}
% \yw{appendix of SGC, GCN comparison}

Though FeatProp is tailored for GCNs, we could also test the effectiveness of our algorithm over other GNN frameworks. Specifically, we compare the methods over a Simplified Graph Convolution (SGC)  \citep{wu2019simplifying} and obtain similar observations. Due to the space limit, we put the detailed results in the appendix.


==> sections/intro.tex <==
\section{Introduction}
Graph Neural Networks (GNN) \citep{kipf2016semi, velivckovic2017graph, hamilton2017inductive, wu2019simplifying} have been widely applied in many supervised and semi-supervised learning scenarios such as node classifications, edge predictions and graph classifications over the past few years. Though GNN frameworks are effective at fusing both the feature representations of nodes and the connectivity information, people are longing for enhancing the learning efficiency of such frameworks using limited annotated nodes.
% In the node classification task, which is the subject we center on, GNNs are shown to have good generalization ability via training with only dozens of annotated nodes. 
This property is in constant need as the budget for labeling is usually far less than the total number of nodes. 
For example, in biological problems where a graph represents the chemical structure \citep{gilmer2017neural} of a certain drug assembled through atoms, it is not easy to obtain a detailed analysis of the function for each atom since getting expert labeling advice is very expensive. On the other hand, people can carefully design a small ``seeding pool'' so that by selecting ``representative'' nodes or atoms as the training set, a GNN can be trained to get an automatic estimation of the functions for all the remaining unlabeled ones.

Active Learning (AL) \citep{settles2009active}, following this lead, provides solutions that select ``informative'' examples as the initial training set. 
While people have proposed various methods for active learning on graphs \citep{bilgic2010active,moore2011active}, active learning for GNN has received relatively few attention in this area. \cite{cai2017active} and \cite{gao2018active} are two major works that study active learning for GNN. 
The two papers both use three kinds of metrics to evaluate the training samples, namely uncertainty, information density, and graph centrality. The first two metrics make use of the GNN representations learnt using both node features and the graph; while they might be reasonable with a good (well-trained) GNN model, the metrics are not informative when the label budget is limited and/or the network weights are under-trained so that the learned representation is not good. On the other hand, graph centrality ignores the node features and might not get the real informative nodes. Further, methods proposed in \cite{cai2017active,gao2018active} only combine the scores using simple linear weighted-sum, which do not solve these problems principally.
% \yw{add a connecting sentence}
% These methods utilize previous active learning and graph metrics to indicate informativeness. Here, the active learning metrics only use the current network representation to compute scores and ignores the graph structure, whereas the graph metrics only use the graph connections and ignore the network representation. 
%Both methods use existing active learning metrics and graph centrality as informativeness scores, 
%and try to find a linear combination of scores to optimize performance. All these methods takes either the node representation or the raw graph structure into account; 
% None of these works have tried to combine the graph structure with node features.
% Active learning under the graph learning setting has received relatively few attention in this area, with the only two 
%\yw{should put in a more thorough literature} 
% The most common approach in AL is uncertainty sampling \citep{settles2009active} where the nodes that the current model is least certain about along with the training phase are selected. Another major stream of AL approaches is the clustering-based selection strategy. Coreset \citep{sener2017active}, as one representative method in this category, generates several anchor points so that each node's feature representation is within a close proximity to one of the anchors. Nodes that are closest to the anchors are selected as the representative initial training set.

% However, existing methods face yet new challenges when applied to the GNN setting\yw{citation}. Given the relatively small size of graphs, a GNN is prune to overfitting issues, and the uncalibrated predictions by a GNN usually do not represent the true informativeness of data points, which deteriorates the effectiveness of uncertainty-based methods. On the other hand, clustering-based approaches like Coreset do consider the relation of nodes through the graph, and therefore fail to identify the central nodes. 
% \yw{bridge the sentence between the prev part} In another aspect, however, being able to consider the GNN framework characteristics can potentially help select nodes that are not only representative of the data distribution but also to the training efficiency of the specific GNN structure.

We propose a method specifically designed for GNN that naturally avoids the problems of methods above\footnote{Our code will be released upon acceptance.}. Our method select the nodes based on node features propagated through the graph structure, making it less sensitive to inaccuracies of representation learnt by under-trained models. Then we cluster the nodes using K-Medoids clustering; K-Medoids is similar to the conventional K-Means, but constrains the centers to be real nodes in the graph.
% We give formal theoretical guarantees on the accuracy that our method can achieve, and conjecture that previous methods cannot achieve such bounds. 
% However, our experiments (see Figure~\ref{fig:main}) show that these existing methods perform similarly to random sampling in most cases when applied to the graph domain. We conjecture that this is because none of these methods expressly consider the downstream classification algorithms (i.e. GNN frameworks) which uses the graph structure to achieve a good performance. As traditional AL settings do not include such graphs, the selected samples therefore might not be representative enough when combined with GNN frameworks. %the same based on features or graphs.
% In this paper we propose a solution to GNN frameworks in the graph learning setting, to address this issue. %to avoid the aforementioned problems of existing methods.
% To the best of our knowledge, there is no previous AL work with the explicit consideration of GNN structures. % \yw{}
% However,
% all of the aforementioned methods are model-agnostic that view the back-end framework (i.e. classification algorithms) as blackboxes: uncertainty sampling only considers the final output while Coreset utilizes node feature representations from the second-to-last layer of the neural network. Performing any framework change will have no influence on these AL methods. In another aspect, however, different GNNs do differ in their structures, and being able to consider the structure characteristics can potentially help select nodes that are not only representative of the data distribution but also to the training efficiency of the specific GNN structure. To the best of our knowledge, there is no previous work that studies AL problems with the explicit model-aware consideration of GNN structures.
% In this work, we present, for the first time, a novel lightweight AL method  specifically designed for the Graph Convolution Network (GCN) \citep{kipf2016semi}, one of the most widely-used GNN structures. 
% Our method performs the node feature propagation succeeded by the K-Means clustering to select representative nodes %over propagated node features and choose the nodes most close to the centers as the training set, 
%  so that the information of the graph structure and the node features are fused in a similar way as the GNN does. 
Theoretical results and practical experiments prove the strength of our algorithm. 
%  We also compare our methods systematically with state-of-the-art AL methods. 
%  The contributions of our work are mainly three-fold: % \yw{}% \yw{rewording of the following contributions}:
\begin{itemize}
    % \item We propose a new AL method, tailored for GCNs, for the node classification task.
    \item We perform a theoretical analysis for our method and study the relation between its classification loss and the geometry of the propagated node features. 
    \item We show the advantage of our method over Coreset \citep{sener2017active} by comparing the bounds. We also conjecture that similar bounds are not achievable if we use raw unpropagated node features. 
    % We also conjecture that previous methods in active graph learning cannot achieve similar bounds.
    %superiority over one existing method -- Coreset 
    \item We compare our method with several AL methods and obtain the best performance over all benchmark datasets.
    % \yx{maybe some visualization?}
\end{itemize}



==> sections/proof.tex <==
\section{Theorem Proofs}
\label{sec:proofs}
\subsection{Proof of Theorem \ref{th:main}}
\newcommand{\networkweight}{\Theta}
% Throughout the proof, we let $z_{i,c}=I(y_i=c)$ be the indicator of label values.
For simplicity, for any model $\model$ let $\modelpred{\model}{i}=(\model(G,X))_i\in \mathbb{R}^C$ be the prediction for node $i$ under input $G,X$, and $\modelpred{\model}{i,c}$ be the $c$-th element of $\modelpred{\model}{i}$ (i.e., the prediction for class $c$). In order to show Theorem \ref{th:main}, we make the following assumptions:\\
\textbf{Assumption 1.} We assume $\algo_0$ overfits to the training data. Specifically, we assume the following two conditions: i) $\algo_0$ has zero training loss on $\selected{0}$; ii) for any unlabeled data $(x_i,x_j)$ with $i\not\in \selected{0}$ and $j\in \selected{0}$, we have $(\algo_0)_{i,y_j}\leq (\algo_0)_{j,y_j}$ and $(\algo_0)_{i,c}\geq (\algo_0)_{j,c}$ for all $c\ne y_j$. The second condition states that $\algo_0$ achieves a high confidence on trained samples and low confidence on unseen samples. We also assume that the class probabilities are given by a ground truth GCN; i.e., there exists a GCN $\gtmodel$ that predicts $\Pr[Y_i=c]$ on the entire training set. 
% achieves a very large prediction at the (known) correct label and a very small prediction at the incorrect values. 
This is a common assumption in the literature, and \citep{du2018gradient} shows that gradient descent provably achieves zero training loss and a precise prediction in polynomial time.\\
% \textbf{Assumption 2.} \\
\textbf{Assumption 2.} We assume that there exists a constant $\alpha$ such that the sum of input weights of every neuron is less than $\alpha$. Namely, we assume $\sum_i|(\networkweight_K)_{i,j}|\leq \alpha$. This assumption is also present in \citep{sener2017active}. We note that one can make $\sum_i|(\networkweight_K)_{i,j}|$ arbitrarily small without changing the network prediction; this is because dividing all input weights by a constant $t$ will also divide the output by a constant $t$.\\
\textbf{Assumption 3.} We assume that ReLU function activates with probability 1/2. This is a common assumption in analyzing the loss surface of neural networks, and is also used in \citep{kawaguchi2016deep,xu2018representation}. This assumption also aligns with observations in practice that usually half of all the ReLU neurons can activate.

With these assumptions in place, we are able to prove Theorem \ref{th:main}.

\textbf{Theorem \ref{th:main} (restated).} Suppose Assumptions 1-3 hold, and the label vector $Y$ is sampled independently from the distribution $y_v\sim \eta(v)$ for every $v\in \nodeset$. Then with probability $1-\delta$ the expected classification loss of $\algo_t$ satisfies
\begin{align}
    \frac{1}{n}l(\algo_0|\graph,\featuremat,\labelvec)\leq& \frac{(\lip+\lossbound)(\alpha/2)^K}{n}\sum_{i=1}^n \min_{j\in \selected{0}}\|(S^KX)_i\nonumber
    \\&-(S^KX)_j\|_2 + \sqrt{\frac{\lossbound\log(1/\delta)}{2n}}.
\end{align}
% We assume i) $\algo_t$ has zero training loss on $\selected{0}$, and  $l$ is Lipschitz with constant $\lip$ and  ii) There exists a constant $\alpha$ such that the sum of input weights of every neuron is less than $\alpha$. iii) ReLU function activates with probability 1/2.
\begin{proof}
Fix $y_j$ for $j\in \selected{0}$ and therefore the resulting model $\algo_0$. Let $i \in \nodeset\setminus \selected{0}$ be any node and $j\in \selected{0}$. We have
\begin{align}
    &\quad\E_{y\sim \eta(i)}\left[l(\modelpred{\almodel}{i},y) \right]\nonumber\\
    &=\sum_{c=1}^C \Pr[Y_i=c]l(\modelpred{\almodel}{i,c},c)\nonumber\\
    % &=\sum_{c=1}^C \Pr[Y_i=c]l(\modelpred{\almodel}{i,c},c)\\
    &=\sum_{c=1}^C \Pr[Y_j=c]l(\modelpred{\almodel}{i,c},c)\nonumber\\
    &\quad+\sum_{c=1}^C \left(\Pr[Y_i=c]-\Pr[Y_j=c]\right)l(\modelpred{\almodel}{i,c},c).\label{eqn:decomp}
\end{align}
For the first term we have 

\begin{align}
    &\quad\sum_{c=1}^C \Pr[Y_j=c]l(\modelpred{\almodel}{i,c},c)\nonumber\\
    &=\sum_{c=1}^C \Pr[Y_j=c]\left[l(\modelpred{\almodel}{i,c},c)-l(\modelpred{\almodel}{j,c},c)\right]\nonumber\\
    & \;\;+\sum_{c=1}^C \Pr[Y_j=c]l(\modelpred{\almodel}{j,c},c)\nonumber\\
    &=\sum_{c=1}^C \Pr[Y_j=c]\left[l(\modelpred{\almodel}{i,c},c)-l(\modelpred{\almodel}{j,c},c)\right]\nonumber\\
    &\leq \lip\sum_{c=1}^C \Pr[Y_j=c]\left|\modelpred{\almodel}{i,c}-\modelpred{\almodel}{j,c}\right|\label{eqn:firstterm_c}
    %\lip\alpha^K \left\|(S^KX)_i-(S^KX)_j\right\|
\end{align}

The last inequality holds from the Lipschitz continuity of $l$. Now from Assumption 1, we have $\modelpred{\almodel}{i,c}\geq \modelpred{\almodel}{j,c}$ for $c\ne Y_j$ and $\modelpred{\almodel}{i,c}\leq \modelpred{\almodel}{j,c}$ otherwise. Now taking the expection w.r.t the randomness in ReLU we have
\begin{align}
    &\quad\E_\sigma[\modelpred{\almodel}{i,c}-\modelpred{\almodel}{j,c}]\nonumber\\
    &=\E_\sigma\left[\sigma((SX^{(K-1)})_i\networkweight^c_K)-\sigma((SX^{(K-1)})_j\networkweight^c_K)\right]\nonumber\\
    &= \frac{1}{2}\E_\sigma\left[(SX^{(K-1)})_i\networkweight^c_K-(SX^{(K-1)})_j\networkweight^c_K\right]\nonumber\\
    &\leq \frac{\alpha}{2}\E_\sigma\left[(SX^{(K-1)})_i-(SX^{(K-1)})_j\right]\nonumber\\
    &\leq \cdots \leq \left(\frac{\alpha}{2}\right)^K \left\|(S^KX)_i-(S^KX)_j\right\|. \label{eqn:boundE}
\end{align}
Here $\E_\sigma$ represents taking the expectation w.r.t ReLU. Now for (\ref{eqn:firstterm_c}) we have
\begin{align*}
    &\E_\sigma\left[\sum_{c=1}^C \Pr[Y_j=c]\left|\modelpred{\almodel}{i,c}-\modelpred{\almodel}{j,c}\right|\right]\\
    =&\E_\sigma\left[\sum_{c\ne Y_j} \Pr[Y_j=c]\left(\modelpred{\almodel}{i,c}-\modelpred{\almodel}{j,c}\right)\right] +\\
    &\; \E_\sigma\left[\Pr[Y_j=y_j]\left(\modelpred{\almodel}{j,y_c}-\modelpred{\almodel}{i,c}\right)\right]\\
    \leq&  \; \sum_{c=1}^C \Pr[Y_j=c] \left(\frac{\alpha}{2}\right)^K \left\|(S^KX)_i-(S^KX)_j\right\|\\
    = & \; \left(\frac{\alpha}{2}\right)^K \left\|(S^KX)_i-(S^KX)_j\right\|.
\end{align*}
The inequality follows from (\ref{eqn:boundE}).
% % original proof
% \begin{align*}
%     l(\modelpred{\almodel}{i,c},c)-l(\modelpred{\almodel}{j,c},c)&\leq \lip|\modelpred{\almodel}{i,c}-\modelpred{\almodel}{j,c}|\\
%     &=\lip\left|\sigma((SX^{(K-1)})_i\networkweight^c_K)-\sigma((SX^{(K-1)})_j\networkweight^c_K)\right|\\
%     &\leq \lip\left|(SX^{(K-1)})_i\networkweight^c_K-(SX^{(K-1)})_j\networkweight^c_K\right|\\
%     &\leq \lip\alpha\left\|(SX^{(K-1)})_i-(SX^{(K-1)})_j\right\|\\
%     &\leq \lip\alpha^2\left\|(S^2X^{(K-2)})_i-(S^2X^{(K-2)})_j\right\|\\
%     &\leq \cdots \leq \lip\alpha^K \left\|(S^KX)_i-(S^KX)_j\right\|.
% \end{align*}
% Here $(M)_i$ is the $i$-th row of matrix $M$, $\networkweight_K^c$ is the $c$-th column of $\networkweight_K$, $\sigma$ is the ReLU activation function. The first inequality follows from Lipschitz property of $l$; the second inequality follows from that ReLU is 1-Lipschitz; the third inequality follows from the definition of $\alpha$; the next few inequalities follows the same process as above.
% \begin{align*}
%     l(\modelpred{\almodel}{i,c},c)-l(\modelpred{\almodel}{j,c},c)&\leq \lip|\modelpred{\almodel}{i,c}-\modelpred{\almodel}{j,c}|\\
%     &=\lip\left|\sigma((SX^{(K-1)})_i\networkweight^c_K)-\sigma((SX^{(K-1)})_j\networkweight^c_K)\right|\\
%     &\leq \lip\left|(SX^{(K-1)})_i\networkweight^c_K-(SX^{(K-1)})_j\networkweight^c_K\right|\\
%     &\leq \lip\alpha\left\|(SX^{(K-1)})_i-(SX^{(K-1)})_j\right\|\\
%     &\leq \lip\alpha^2\left\|(S^2X^{(K-2)})_i-(S^2X^{(K-2)})_j\right\|\\
%     &\leq \cdots \leq \lip\alpha^K \left\|(S^KX)_i-(S^KX)_j\right\|.
% \end{align*}


% Therefore
% \begin{align*}
%     \sum_{c=1}^C \Pr[Y_j=c]l(\modelpred{\almodel}{i,c},c)&=\sum_{c=1}^C \Pr[Y_j=c]\left[l(\modelpred{\almodel}{i,c},c)-l(\modelpred{\almodel}{j,c},c)\right]\\
%     & \;\;+\sum_{c=1}^C \Pr[Y_j=c]l(\modelpred{\almodel}{j,c},c)\\
%     &=\sum_{c=1}^C \Pr[Y_j=c]\left[l(\modelpred{\almodel}{i,c},c)-l(\modelpred{\almodel}{j,c},c)\right]\\
%     &\leq \lip\alpha^K \left\|(S^KX)_i-(S^KX)_j\right\|
% \end{align*}
% The second equality follows from the fact that $\almodel$ has zero training loss.

Now for the second loss in (\ref{eqn:decomp}) we use the property that $\gtmodel$ computes the ground truth:
\begin{align*}
    &\left(\Pr[Y_i=c]-\Pr[Y_j=c]\right)l(\modelpred{\almodel}{i,c},c)\\
    =&\left(\modelpred{\gtmodel}{i,c}-\modelpred{\gtmodel}{j,c}\right)l(\modelpred{\almodel}{i,c},c)
\end{align*}
We now use the fact that ReLU activates with probability $1/2$, and compute the expectation:
\begin{align*}
    &\quad\E_{\sigma}\left[\left(\modelpred{\gtmodel}{i,c}-\modelpred{\gtmodel}{j,c}\right)l(\modelpred{\almodel}{i,c},c)\right]\\
    &=\E_{\sigma}\left[\left(\modelpred{\gtmodel}{i,c}-\modelpred{\gtmodel}{j,c}\right)\right]l(\modelpred{\almodel}{i,c}\\
    &=\left(\E_{\sigma}\left[\modelpred{\gtmodel}{i,c}\right]-\E_{\sigma}\left[\modelpred{\gtmodel}{j,c}\right]\right)l(\modelpred{\almodel}{i,c}\\
    &=\frac{1}{2^K}\left((S^KX)_i-(S^KX)_j\right)\networkweight_1\networkweight_2\cdots \networkweight^c_{K}l(\modelpred{\almodel}{i,c}\\
    &\leq \lossbound\left(\frac{\alpha}{2}\right)^K \|(S^KX)_i-(S^KX)_j\|.
\end{align*}
Here $\E_{\sigma}$ means that we compute the expectation w.r.t randomness in $\sigma$ (ReLU) in $\gtmodel$. The last inequality follows from definition of $\alpha$, and that $l\in [-\lossbound,\lossbound]$.

Combining the two parts to (\ref{eqn:decomp}) and let $j=\argmin \|(S^KX)_i-(S^KX)_j\|$, we obtain
\begin{align}
  \E_{y\sim \eta(i),\sigma}\left[l(\modelpred{\almodel}{i},y)\right]\leq&  (\lip+\lossbound)(\alpha/2)^K \min_j\|(S^KX)_i\nonumber\\
  &-(S^KX)_j\|.  \label{eqn:bound_El}
\end{align}

Now notice that
\begin{align}
    l(\algo_0|\graph,\featuremat,\labelvec)&=\sum_{i\in V\setminus \selected{0}} l(\modelpred{\almodel}{i},y_i)+\sum_{j\in \selected{0}} l(\modelpred{\almodel}{j},y_j)\nonumber\\
    &=\sum_{i\in V\setminus \selected{0}} l(\modelpred{\almodel}{i},y_i).\label{eqn:reduce_l}
\end{align}
\newcontent{Consider the following process: we first get $G,X$ (fixed data) as input, which induces $\eta(i)$ for $i\in [n]$. Note that $\gtmodel$ gives the ground truth $\eta(i)$ for every $i$ so distributions $\eta(i)\equiv\eta_{X,G}(i)$ are fixed once we obtain $G,X$ \footnote{To make a rigorous argument, we get the activation of $\gtmodel$ in this step, meaning that we pass through the randomness of $\sigma$ in $\gtmodel$.}. Then the algorithm $\algo$ choose the set $\selected{0}$ to label. After that, we randomly sample $y_j\sim \eta(j)$ for $j\in \selected{0}$ and use the labels to train model $\algo_0$. At last, we randomly sample $y_i\sim \eta(i)$ and obtain loss $l(\algo_0|\graph,\featuremat,\labelvec)$. Note that the sampling of all $y_i$ for $i\in V\setminus \selected{0}$ is after we fix the model $\algo_0$, and knowing exact values of $y_j$ for $j\in \selected{0}$ does not give any information of $y_i$ (since $\eta(i)$ is only determined by $G,X$). 
Now we use Hoeffding's inequality (Theorem {\ref{thm:hoefdding}}) with $Z_i=l(\modelpred{\almodel}{i},y_i)$; we have $-L\leq Z_i\leq L$ by our assumption, and recall that $|V\setminus \selected{0}|=n-b$. Let $\delta$ be the RHS of ({\ref{eqn:hoeffding}}), we have that with probability $1-\delta$, }
\begin{align}
&\quad\frac{1}{n-b}\sum_{i\in V\setminus \selected{0}}l(\modelpred{\almodel}{i},y_i) \nonumber\\&- \frac{1}{n-b}E_{y\sim \eta(i),\sigma}\left[l(\modelpred{\almodel}{i},y_i)\right]
\leq \sqrt{\frac{\lossbound\log(1/\delta)}{2(n-b)}}.
\end{align}
\newcontent{Now plug in ({\ref{eqn:bound_El}}), multiply both sides by $(n-b)$ and rearrange. We obtain that}
\begin{align}
    \sum_{i\in V\setminus \selected{0}}l(\modelpred{\almodel}{i},y_i)\leq &\sum_{i\in V\setminus \selected{0}} (\lip+\lossbound)(\alpha/2)^K \min_j\|(S^KX)_i\\&-(S^KX)_j\|+ \sqrt{\frac{\lossbound\log(1/\delta)(n-b)}{2}}.\label{eqn:boundloss_2}
\end{align}
\newcontent{Now note that since the random draws of $y_i$ is completely irrelevant with training of $\algo_0$, we can also sample $y_i$ together with $y_j$ for $j\in \selected{0}$ after receiving $G,X$ and before the training of $\algo_0$ ($\algo$ does not have access to the labels anyway). So ({\ref{eqn:boundloss_2}}) holds for the random drawings of all $y$'s. Now divide both sides of ({\ref{eqn:boundloss_2}}) by $n$ and use ({\ref{eqn:reduce_l}}), we have}
\begin{align*}
    \frac{1}{n}l(\algo_0|\graph,\featuremat,\labelvec)\leq& \frac{(\lip+\lossbound)(\alpha/2)^K}{n}\sum_{i=1}^n \min_{j\in \selected{0}}\|(S^KX)_i\\
    &-(S^KX)_j\|_2 + \sqrt{\frac{\lossbound\log(1/\delta)(n-b)}{2n^2}}\\
    \leq& \frac{(\lip+\lossbound)(\alpha/2)^K}{n}\sum_{i=1}^n \min_{j\in \selected{0}}\|(S^KX)_i\\
    &-(S^KX)_j\|_2 + \sqrt{\frac{\lossbound\log(1/\delta)}{2n}}.
\end{align*}

% Further , sum over all $i\in \nodeset\setminus\selected{0}$ and use Hoeffding's inequality  based on $l\in [-\lossbound,\lossbound]$ gives
% \[\frac{1}{n}l(\algo_0|\graph,\featuremat,\labelvec)\leq \frac{(\lip+\lossbound)(\alpha/2)^K}{n}\sum_{i=1}^j \min_j\|(S^2X)_i-(S^2X)_j\|_2 + \sqrt{\frac{\lossbound\log(1/\delta)}{2n}} \]

\end{proof}

\subsection{Proof of Theorem \ref{thm:bound_center} }


The same proof as Theorem \ref{th:main} applies for Theorem \ref{thm:bound_center} using the max of distances instead of averaging.
We therefore omit the details here.


==> sections/related.tex <==
\section{Related Works}
% \yx{this section can be shorter and merged; let us decide later.}
% \yw{comparison between two existing AL on graph algorithms should be mentioned.}
% \subsection{Active Learning}
\textbf{Active Learning (AL)} aims at interactively choosing data points from the training pool to maximize model performances, and has been widely studied both in theory \citep{hanneke2014theory} and practice \citep{Shen_2017}. Recently, \cite{sener2017active} proposes to compute a Coreset over the last-layer activation of a convolutional neural network. The method is designed for general-purpose neural networks, and does not take the graph structure into account.
%A central problem in AL is the tradeoff between exploration and exploitation: During exploration, we would like to select most representative training samples in the training set. This has resulted in clustering-based methods \citep{5670014,nguyen2004active,bodo2011active, DBLP:journals/jmlr/TsangKC05}. For exploitation, the algorithm aims to find the data point that results in the maximal information gain. Popular methods in this regime include model uncertainty \citep{yang2016active} and margin to the decision boundary \citep{DBLP:journals/jmlr/TongK01}. Recently there have been methods that try to combine exploitation and exploration. For example, Sener et al.\citep{sener2017active} computes a Coreset cover over the last-layer activations of a convolutional neural network. 
%However such methods are mostly model-agnostic which put no special attention for GNN structures that can potentially be helpful.
% meaning that changing the underlining structure of the neural network will do no influence on the AL procedures/hyperparameters.
%We discuss the relation between our method and Coreset in Section \ref{sec:not_coreset}. 

%Except for the AL method dealing with data on the normal Euclidean space, s
Early works on AL with graph-structured data \citep{DBLP:conf/colt/DasarathyNZ15,DBLP:conf/cvpr/AodhaCKB14} study non-parametric classification models with graph regularization. More recent works analyze active sampling under the graph signal processing framework \citep{GSP}. However, most of these works have focused on the denoising setting where the signal is smooth over the graphs and labels are noisy versions of node features. Similarly, optimal experimental design \citep{Expdesign_book,DBLP:journals/corr/abs-1711-05174} can also apply to graph data but primarily deals with linear regression problems, instead of nonlinear classification with discrete labels. %\yw{Move sentence to previous part}
%where it is shown that passive experimental design can leverage the graph structure well and active sampling does not buy further improvement over passive experimental design.  



% how to measure the ``informativeness'' of the unlabeled data. In general, people usually tackle this challenge from two aspects: either through prediction uncertainty of the current model to the data or through the data expressiveness along. 

% \begin{itemize}
%     \item \textbf{Uncertainty:} centers on 
%     \item \textbf{Data expressiveness:} Corset: The Coreset method centers on expressiveness; more on this in; many clustering methods belong to this category. Section~\ref{sec:not_coreset}. Considers CNN, but not GNN.

% \end{itemize}
% \subsection{Graph Neural Network}
\textbf{Graph Neural Networks (GNNs)}  \citep{hamilton2017inductive,velivckovic2017graph,kipf2016semi} are the emerging frameworks in the recent years when people try to model graph-structured data. Most of the GNN variants follow a multi-layer paradigm. In each layer, the network performs a message passing scheme, so that the feature representation of a node in the next layer could be some neighborhood aggregation from its previous layer. The final feature of a single node thus comprises of the information from a multi-hop neighborhood, and is usually universal and ``informative'' to be used for multiple tasks. % Noticeably, the layers could also be combined with pooling operations so that the network could output a single vectorized representation in the final layer which can be assumed to obtain a summary of the whole graph. Specifically, such GNN structures are shown empirically to achieve state-of-the-art performances in tasks including node classification, edge prediction and graph classifications.  
Recent works show the effectiveness of using GNNs in the AL setting. \cite{cai2017active}, for instance, proposes to linearly combine uncertainty, graph centrality and information density scores and obtains the optimal performance. \cite{gao2018active} further improves the result by using learnable combination of weights with multi-armed bandit techniques. Instead of combining different metrics, in this paper, we approach the problem by clustering propagated node features. We show that our one-step active design outperforms existing methods based on learnt network represenations, in the small label setting, while not degrading in performance for larger amounts of labeled data.
% Our work improves on these results by using propagated node features and K-Medoids clustering.
% As discussed above, 
% their metrics considers the network representation and graph structure separately,  while our metric can take both into account.
% cannot take information from features and graph structure into account jointly. 
% \yw{to be modified}
% However, nearly all of the works with GNNs proceed these problems in a supervised/semi-supervised way, while no active sampling is considered. 

% Although earlier works have studied active learning on graphs \citep{DBLP:conf/colt/DasarathyNZ15,DBLP:conf/cvpr/AodhaCKB14},
% To the best of our knowledge no previous works have studied AL with explicit consideration of GNN structures, which is one of the key contributions in our work.

% It is important to note that though cluster-based active learning has been studied in previous works \citep{nguyen2004active,bodo2011active}, there is no explicit model-aware consideration/analysis of any of the aforementioned approaches with GNN frameworks, which is one of the key contribution in our work.


==> sections_iclr/approach.tex <==
\newcommand{\graph}{G}
\newcommand{\nodeset}{V}
\newcommand{\node}{v}
\newcommand{\feature}{x}
\newcommand{\labely}{y}
\newcommand{\featuremat}{X}
\newcommand{\labelvec}{Y}
\newcommand{\numclass}{C}
\newcommand{\featurespace}{\gX}
\newcommand{\labelspace}{\gY}
\newcommand{\numtrain}{n}\newcommand{\model}{\gM}
\newcommand{\selected}[1]{\mathbf{s}^{#1}}
\newcommand{\algo}{\gA}

\section{Preliminaries}



% \subsection{Problem Definition}

In this section, we describe a formal definition for the problem of graph-based active learning under the node classification setting and introduce a uniform set of notations for the rest of the paper. 
% Specifically, we are interested in a $C$ class classification problem, where the observations $(X, Y, G)$ denotes features drawn from compact space $\gX$, labels from space $\gY = \{1, \dots, C\}$ and the linkage information (graph) $G$. 
% Naturally, one can not assume the independence of nodes as their neighboring information does suggest certain degree of correlation. However, to cast the problem into a similar setting as the traditional classification problem, let us assume that there exists a prior (infinite) graph $G_0$ along with a probability space $P_0$ and vertex set $V_0$, so that the observation $G$ is an induced graph from $G_0$ via $P_0$ and each node can be viewed as i.i.d. samples of $V_0$.


We are given a large graph $\graph=(\nodeset,E)$, where each node $\node\in \nodeset$ is associated with a feature vector $\feature_\node \in \featurespace\subseteq \R^d$, and a label $\labely_\node \in \labelspace= \{1,2,...,\numclass\}$. Let $\nodeset=\{1,2,...,n\}$, we denote the input  features as a matrix $X\in \R^{\numtrain\times d}$, where each row represents a node, and the labels as a vector $\labelvec=(\labely_1,...,\labely_\numtrain)$.
We also consider a loss function
$l(\model | \graph, \featuremat, \labelvec)$ that computes the loss over the inputs $(\graph, \featuremat, \labelvec)$ for a model $\model$ that maps $\graph, \featuremat$ to a prediction vector $\hat{\labelvec} \in \labelspace^{\numtrain}$. 

Following previous works on GNN\citep{cai2017active,hamilton2017inductive}, we consider the inductive learning setting; i.e., a small part of $\labelvec$ is revealed to the algorithm, and we wish to minimize the loss on the whole graph $l(\model | \graph, \featuremat, \labelvec)$.
% $\graph\times \featurespace\rightarrow \labelspace$ (here we slightly abuse the notation to denote that $\graph$ is also an input to $\model$). 
Specifically, an active learning algorithm $\algo$ is initially given the graph $\graph$ and feature matrix $ \featuremat$. 
In step $t$ of operation, it selects a subset $\selected{t}\subseteq [\numtrain]=\{1,2,...,\numtrain \}$, 
and obtains $\labely_i$ for every $i\in \selected{t}$. 
We assume $\labely_i$ is drawn randomly according to a distribution $\mathbb{P}_{y|x_i}$ supported on $\labelspace$; we use $\eta_c(v)=\Pr[y=c|v]$ to denote the probability that $y=c$ given node $v$, and $\eta(v)=(\eta_1(v),...,\eta_C(v))^T$.
Then $\algo$ uses $\graph, \featuremat$ and $\labely_i$ for  $i\in \selected{0}\cup \selected{1}\cup \cdots\cup \selected{t}$ as the training set to train a model, using training algorithm $\model$. The trained model is denoted as $\model_{\algo_t}$. If $\model$ is the same for all active learning strategies, we can slightly abuse the notation $\algo_t= \model_{\algo_t}$ to emphasize the focus of active learning algorithms. A general goal of active learning is then to minimize the loss under a given budget $b$:
\begin{equation}
    \min_{\selected{0}\cup \cdots\cup \selected{t}} \E[l(\algo_t|\graph, \featuremat, \labelvec)] \label{eqn:target}
\end{equation}
where the randomness is over the random choices of $\labelvec$ and $\algo$.
%As $\model$ has multiple choices, 
We focus on $\model$ being the Graph Neural Networks and their variants elaborated in detail in the following part.

\subsection{Graph Neural Network Framework}
% \textbf{Graph Neural Network Framework}
% \yx{define S.}
Graph Neural Networks define a multi-layer feature propagation process similar to Multi-Layer Perceptrons (MLPs). Denote the $k$-th layer representation matrix of all nodes as $\featuremat^{(k)}$, and $\featuremat^{(0)}\in \R^{n\times d}$ are the input node features. Graph Neural Networks (GNNs) differ in their ways of defining the recursive function $f$ for the next-layer representation:
\begin{align}
	\featuremat^{(k+1)}&\leftarrow f(\featuremat^{(k)};G,\Theta_k),
\end{align}
where $\Theta_k$ is the parameter for the $k$-th layer. Naturally, the input $\featuremat$ satisfies $\featuremat^{(0)}=\featuremat$ by definition.
\textbf{Graph Convolution Network (GCN)}.
A GCN \citep{kipf2016semi} has a specific form of the function $f$ as:
\begin{align}
	\featuremat^{(k+1)}&\leftarrow \text{ReLU}(S\featuremat^{(k)}\Theta_k),
\end{align}
where ReLU is the element-wise rectified-linear unit activation function \citep{nair2010rectified}, $\Theta_k$ is the parameter matrix used for transforming the size of feature representations to a different dimension and $S$ is the normalized adjacency matrix. Specifically, $S$ is defined as:
\begin{align}
    S=(I+D)^{-\frac{1}{2}}(A+I)(I+D)^{-\frac{1}{2}},
\end{align} where $A$ is the original adjacency matrix associated with graph $G$ and $D$ is the diagonal degree matrix of $A$. Intuitively, this operation updates node embeddings by the aggregation of their neighbors. The added identity matrix $I$ (equivalent to adding self-loops to $G$) acts in a similar spirit to the residual links \citep{he2016deep} in MLPs that bypasses shallow-layer representations to deep layers. By applying this operation in a multi-layer fashion, a GCN encourages nodes that are locally related to share similar deep-layer embeddings and prediction results thereafter.

For the classification task, it is normal to stack a linear transformation along with a softmax function to the representation in the final layer, so that each class could have a prediction score. That is,
\begin{align}
    \hat{Y}&=\text{softmax}(\featuremat^{(K)}\Theta_K),
\end{align}
where $\text{softmax}(\vx)=\exp(\vx)/\sum_{c=1}^C \exp(x_c)$ which makes the prediction scores have unit sum of 1 for all classes, and $K$ is the total number of layers. We use the GCN structure as the fixed unified model $\model$ for all the following discussed AL strategies $\algo$.% \yw{}
% \yw{note that data points are no-longer independent as the normalized adjacency matrix mingles their feature representations.}


% the GCN model, and each class-specific conditional probability $\eta_c(\vx)=p(y=c|\vx)$ to be $\lambda^\eta$-Lipschitz continuous for all $c$.


\section{Active Learning Strategy \& Theoretical Analysis}
% \begin{algorithm}[ht]
% 	\caption{Propagated Embedding Selection}
% 	\label{algo:K-Medoids}
% 	\begin{algorithmic}[1]        
% 		\Require{Representation matrix $\featuremat$, normalized adjacency matrix $S$ and a budget $b$}
% 		\State Compute propagated embeddings as $\featuremat'=S^k \featuremat$ \Comment{$k$ is the number of layers in the GCN}
% 		\State Perform K-Medoids over $\featuremat'$ with $b$ centers
% 		\State Select $\selected{}$ to be nodes that are closest to these centers\\
% 		\Return{$\selected{}$}
% 	\end{algorithmic}
% \end{algorithm}


% \yy{I rewrote this paragraph:}
%Traditionally, active learning choose labels in a purely sequential fashion, i.e., each time $\algo$ only queries one label, 
Traditionally, active learning algorithms choose one instance at a time for labeling, i.e.,
with $|\selected{t}|=1$. 
% However, such behavior is infeasible in practice mainly because of two reasons: i) Modern datasets contain very large numbers of points and it can be extremely time-consuming if we collect the labels one by one; ii) It is also infeasible to retrain the network at each step during the training process since it takes a long time. 
However, for modern datasets where the numbers of training instances are very large, it would be extremely costly if we re-train the entire system each time when a new label is obtained.
Hence we focus on the %\textit{one-step} 
% \yy{\textit{mini-batch}}
``batched'' one-step active learning setting \citep{contardo2017meta}, and select the informative nodes once and for all when the algorithm starts.
This is also called the \textit{optimal experimental design} in the literature \citep{Expdesign_book,DBLP:journals/corr/abs-1711-05174}. 
Aiming to select the $b$ most representative nodes as the batch, our target (\ref{eqn:target}) becomes:
\begin{equation}
    \min_{|\selected{0}|\leq b} \E[l(\algo_0|\graph, \featuremat, \labelvec)]. 
\end{equation}
%that aims at selecting 
% Our algorithm therefore focuses on the best method to select 
%the most representative points in $\nodeset$. 
% \yy{I rewrote the next paragraph, too:}
The node selection algorithm is described in Section~\ref{sec:pes}, followed by the loss bound analysis in Section~\ref{sec:pes_analysis}, and the comparison with a closely related algorithm (K-Center in Coreset \citep{sener2017active}) in Section~\ref{sec:not_coreset}. 
%In Section~\ref{sec:pes},  we give our \yw{Node Feature Propagation Selection} strategy, and present its theoretical analysis in Section~\ref{sec:pes_analysis}. Then, we give a comparison with the previous Coreset method in Section~\ref{sec:not_coreset}.


% \subsection{Propagated Embedding Selection with K-Medoids Clustering
\definecolor{my_blue}{HTML}{7e80fc}

\subsection{Node Selection via Feature Propagation and K-Medoids Clustering%\yw{revisit this name in the context}
}
\label{sec:pes}
\begin{algorithm}[ht]
	\caption{Active Learning with Distance-based Clustering}
	\label{algo:K-Medoids}
	\begin{algorithmic}[1]        
		\Require{Node representation matrix $\featuremat$, graph structure matrix $G$ and budget $b$}
		\State Compute a distance function $d_{\featuremat, \graph}(\cdot,\cdot): \nodeset\times \nodeset \rightarrow \R $\label{alg:line:dist} \hfill \textcolor{my_blue}{\# for FeatProp: use Eqn. (\ref{eqn:dist})} %\yw{clearer notation}
% 		\State Compute propagated embeddings as $\featuremat'=S^k \featuremat$ \Comment{$k$ is the number of layers in the GCN}
% 		\State Perform K-Medoids over $d_{X,G}$ with $b$ centers\label{alg:line:kmean}
		\State Perform clustering using $d_{X,G}$ with $b$ centers\label{alg:line:kmean} \hfill \textcolor{my_blue}{\# for FeatProp: use K-Medoids}
		\State Select $\selected{}$ to be the centers
		\State Obtain labels for $v\in \selected{}$ and train model $\model$
		\Ensure{Model $\model$}
		\end{algorithmic}
\end{algorithm}

% \yy{Yuexin: Please re-order the paragraphs below: first, introduce the distance matrix, and then applies K-Medoids to the matrix and selects the $b=k$ centroids.}

% Our algorithm (Algorithm \ref{algo:K-Medoids}) acts in two steps: 
We describe a generic active learning framework using distance-based clustering in Algorithm \ref{algo:K-Medoids}. It acts in two major steps:
1) computing a distance matrix or function $d_{X,G}$ using the node feature representations $X$ and the graph structure $G$; 2) applying clustering with $b$ centers over this distance matrix, and from each cluster select the node closest to the center of the cluster. 
After receiving the labels (given by matrix $Y$) of the selected nodes, we train a graph neural network, specifically GCN, based on $X, G$ and $Y$ for the node classification task.  
% The procedure is described in detail in Algorithm~\ref{algo:K-Medoids}. 
Generally speaking, different options for the two steps above would yield different performance in the down-stream prediction tasks; we detail and justify our choices below and in subsequent sections.
% which we will analyze theoretically in Section~\ref{sec:not_coreset} and examine empirically in Section~\ref{sec:exp_res}.

% Here, we discuss a \yw{direct} yet effective design choice for these consecutive procedures.

% We consider a simple K-Medoids based active learning algorithm, presented in Algorithm \ref{algo:K-Medoids}; we first compute a distance matrix $d_{X,G}$ based on the input, and run $k$-MedoidK-Meanrithm on the distance matrix to select $b$ centers. 

%Note that the distance is fully defined by the input feature $X$ and the graph structure $G$, and early trials in the general active learning setting
\textbf{Distance Function.} Previous methods \citep{sener2017active,cai2017active,gao2018active} commonly use network representations to compute the distance, i.e., $d_{X,G}(v_i,v_j)=\|(X^{(k)})_i- (X^{(k)})_j\|_2$ for some specific $k$. While this can be helpful in a well-trained network, the representations are quite inaccurate in initial stages of training and such distance function might not select the representatitive nodes.
% Note that our distance matrix depends on both the node features in $X$ and the graph structure in $G$, while traditional active learning strategies only use $X$ but do not take $G$ into consideration \citep{DBLP:journals/jmlr/BodoMC11,sener2017active}.
%For example, %It only remains to specify the distance matrix $d_{X,G}$. 
%previous methods suggest using L2 distance\citep{sener2017active} or kernel methods \citep{DBLP:journals/jmlr/BodoMC11} over $X$ alone. % These methods cannot take $G$ into account. 
% \yy{I reworded the next}:
%Here, we adopt a direct yet effective design choice for these consecutive procedures. That is, 
Differently, we define the pairwise node distance using the $L_2$ norm of the difference between the corresponding
%for distance $d_{G,X}$ we propose to use L2 over the 
propagated node features: 
\begin{align}
    d_{X,G}(v_i,v_j)=\|(S^KX)_i- (S^KX)_j\|_2, \label{eqn:dist}
\end{align} 
% \textcolor{red}{AS: is this $S^K$ same as $S^k$? Otherwise define what K means.}
where $(M)_i$ denotes the $i$-th row of matrix $M$, and recall that $K$ is the total number of layers. Intuitively, this removes the effect of untrained parameters on the distance, while still taking the graph structure into account.
% \yx{I changed the order of these sentences}
%And for the clustering sub-routine, 
% Intuitively, the propagated features in our approach act as the surrogates of the GCN hidden representations. 

\textbf{Clustering Method.} Two commonly used methods are K-Means \citep{cai2017active,gao2018active} and K-Center \citep{sener2017active}\footnote{For a group of nodes, K-Center problem aims to find a $\delta$-cover with at most $k$ nodes for smallest possible $\delta$.}. We propose to apply the K-Medoids clustering. K-Medoids problem is similar to K-Means, but the center it selects must be real sample nodes from the dataset. This is critical for active learning, since we cannot try to label the unreal cluster centers produced by K-Means.
Also, we show in Section \ref{sec:not_coreset} that K-Medoids can obtain a more favorable loss bound than K-Center.
% to the distance matrix, where each row is treated as the vector representation of each node. % \yy{I rewrote the next paragraph;}
%We call our algorithm Propagated Embedding Selection (PES) as $S^kX$ reflects the propagation characteristics of the input features between locally-connected nodes.
%Notably, % each used option has its own reason 
%\yw{each option is chosen based on its intuitive yet provable characteristics}. Roughly speaking, 
% The K-Medoids clustering
%can be proved to derive a 
% yields a tighter loss bound than K-Center, the clustering method employed by \cite{sener2017active}, as we justify theoretically in the next two sections. 
% After receiving the labels (given by matrix $Y$) of the selected nodes, we train a graph neural network, specifically GCN, based on $X, G$ and $Y$ for the node classification task.  

We call our method \textit{FeatProp}, to emphasize the active learning strategy via node feature propagation over the input graph, which is the major difference from other node selection methods. 
% We specify our choices for distance function and clustering method i
% (Section~\ref{sec:exp_res}).


\subsection{Theoretical Analysis of Classification Loss Bound}
\label{sec:pes_analysis}

\newcommand{\gtmodel}{\model^*}
\newcommand{\almodel}{\algo_0}
\newcommand{\modelpred}[2]{(#1)_{#2}}
\newcommand{\lip}{\lambda}
\newcommand{\lossbound}{L}
%In this section we give theoretical justification on using L2 over propagated embedding as distance function. Basically, we use 
Recall that we use $\|(S^KX)_i- (S^KX)_j\|_2$ to approximate the pairwise distances between the hidden representations of nodes in GCN.   
% \yy{I am not sure your statement here is convincing so I delete it.}
%This means that we can obtain a small classification error for the trained GCN if the error for these surrogate representations is also small \yw{rephrase}. 
Intuitively, representation $S^KX$ resembles the output of a simplified GCN  \citep{wu2019simplifying} by dropping all activation functions and layer-related parameters in the original structure, which introduces a strong inductive bias.
% (thus with small variance due to bias-variance tradeoff). 
In other words, the selected nodes could possibly contribute to the stabilization of model parameters during the training phase of GCN. The following theorem formally shows that using K-Medoids with propagated features can lead to a low classification loss:
\begin{theorem}[informal]
\label{th:main}
Suppose that the label vector $Y$ is sampled independently from the distribution $y_i\sim \eta(i)$, and the loss function $l$ is bounded by $[-\lossbound,\lossbound]$. Then under mild assumptions, there exists a constant $c_0$ such that with probability $1-\delta$ the expected classification loss of $\algo_t$ satisfies
\begin{equation}
    \frac{1}{n}l(\algo_0|\graph,\featuremat,\labelvec)\leq \frac{c_0}{n}\sum_{i=1}^n \min_{j\in \selected{0}}\|(S^KX)_i-(S^KX)_j\|_2 + \sqrt{\frac{\lossbound\log(1/\delta)}{2n}} \label{eqn:bound_kmeans}
\end{equation}
\end{theorem}
To understand Theorem \ref{th:main}, notice that the first term $\sum_{i=1}^n \min_{j\in \selected{0}}\|(S^KX)_i-(S^KX)_j\|_2$ is exactly the target loss of K-Medoids (sum of point-center distances), and the second term $\sqrt{\frac{\lossbound\log(1/\delta)}{2n}}$ quickly decays with $n$, where $n$ is the total number of nodes in graph $G$. Therefore the classification loss of $\almodel$ on the entire graph $G$ is mostly dependent on the K-Medoids loss. In practice, we can utilize existing robust initialization algorithms such as Partitioning Around Medoids (PAM) to 
%\yx{\sout{boost the performance.} 
approximate the optimal solution for K-Medoids clustering.

% \begin{wrapfigure}{r}{0.4\textwidth}
% % \begin{wrapfigure}{r}{0pt}
%   \begin{center}
%     \includegraphics[width=0.4\textwidth]{vis.pdf}
%   \end{center}
%   \caption{Visualization of Theorem~\ref{th:main}. Consider the set of selected points \textcolor{blue}{$\selected{}$} and the remaining points in the dataset \textcolor{red}{$[\numtrain]\backslash \selected{}$}. It suggests from our theorem that the K-Medoids paradigm gives a bound of $\gO(\sum_i d_i/n)+\gO(\sqrt{\frac{1}{n}})$ while K-Center (Section~\ref{sec:not_coreset}) shows $\gO(\max_i d_i)+\gO(\sqrt{\frac{1}{n}})$, which is looser than the former one.}
%     \label{fig:vis}
% \end{wrapfigure}


The assumptions we made in Theorem \ref{th:main} are pretty standard in the literature, and we illustrate the details in the appendix. While our results share some common characteristics with Sener et al.\citep{sener2017active}, our proof is more involved in the sense that it relates to the translated features $\|(S^KX)_i-(S^KX)_j\|_2$ instead of the raw features $\|(X)_i-(X)_j\|_2$. In fact, we conjecture that using raw feature clustering selection for GCN will not result in a similar bound as in (\ref{eqn:bound_kmeans}): this is because GCN uses the matrix $S$ to diffuse the raw features across all nodes in $\nodeset$, and the final predictions of node $i$ will also depend on its neighbors as well as the raw feature $(X)_i$.
% Note that relating the loss to propagated features rather than raw features is desirable, as the latter one without the consideration of graph structures will usually result in a worse performance.
% In fact, using raw feature clustering instead of the propagated features will not result in a bounded classification loss for GCN, because GCN uses the matrix $S$ to diffuse the features across all nodes in $\nodeset$. 
We could see a clearer comparison in practice in Section~\ref{sec:exp_res}.
% \yw{Intuitively, this suggests that we minimize over the summation of point-center distances.}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.5\linewidth]{vis.pdf}
    \caption{Visualization of Theorem~\ref{th:main}. Consider the set of selected points \textcolor{blue}{$\selected{}$} and the remaining points in the dataset \textcolor{red}{$[\numtrain]\backslash \selected{}$}. 
    K-Medoids corresponds to the mean of all red segments in the figure, whereas K-Center corresponds to the max of all red segments in the figure.
%    	It suggests from our theorem that the K-Medoids paradigm gives a bound of $\gO(\sum_i d_i/n)+\gO(\sqrt{\frac{1}{n}})$ while K-Center (Section~\ref{sec:not_coreset}) shows $\gO(\max_i d_i)+\gO(\sqrt{\frac{1}{n}})$, which is looser than the former one.
    }
    \label{fig:vis}
\end{figure}

\newcommand{\coversize}{d}
\subsection{Why not K-Center}
\label{sec:not_coreset}
In this subsection we provide justifications on using the K-Medoids clustering method as opposed to Coreset \citep{sener2017active}. The Coreset approach aims to find a $\delta$-cover of the training set. In the context of using propagated features, this means solving
\begin{align}
\delta=\min_{|\selected{0}|\leq b}\max_i \min_{j\in \selected{0}} d_{\featuremat, \graph}(\node_i, \node_j) =  \min_{|\selected{0}|\leq b}\max_i \min_{j\in \selected{0}} \|(S^KX)_i-(S^KX)_j\|_2 \label{eqn:bound_cover}
\end{align}


We can show a similar theorem as Theorem \ref{th:main} for the Coreset approach:
\begin{theorem}\label{thm:bound_center}
	Under the same assumptions as in Theorem \ref{th:main}, with probability $1-\delta$ the expected classification loss of $\algo_t$ satisfies 
	 \begin{equation}
	\frac{1}{n}l(\algo_0|\graph,\featuremat,\labelvec)\leq c_0\max_i \min_{j\in \selected{0}} \|(S^KX)_i-(S^KX)_j\|_2 + \sqrt{\frac{\lossbound\log(1/\delta)}{2n}}
	%  \frac{1}{n}\sum_{i=1}^n \min_{j\in \selected{0}}\|(S^KX)_i-(S^KX)_j\|_2\leq \. 
	\end{equation}
\end{theorem}

Let $d_i = \min_{j\in \selected{0}} \|(S^KX)_i-(S^KX)_j\|_2$. It is easy to see that RHS of Eqn. (\ref{eqn:bound_kmeans}) is smaller than RHS of Eqn. (\ref{eqn:bound_cover}), since $\frac{1}{n}\sum_{i=1}^n d_i\leq \max_i d_i$. In other words, K-Medoids can obtain a better bound than the K-Center method (see Figure \ref{fig:vis} for a graphical illustration). We observe superior performance of K-Medoid clustering over K-Center clustering in our experiments as well (see Section \ref{sec:exp_res}).

% In fact, our method can also apply to the standard neural networks analyzed in \citep{sener2017active}, and it is interesting to analyze the effect of replacing K-Center with K-Medoids for image classification tasks in the future work.

%Besides the propagated features used to compute centers, another important factor of our algorithm is the K-Medoids clustering. The most related work to our center finding procedure is the K-Center approach in Coreset \citep{sener2017active}, that tries to minimize
%  as opposed to the K-Center option: minimizing 
% the largest point-center distance: 
% \begin{align}
% \min_{|\selected{0}|\leq b}\max_i \min_{j\in \selected{0}} d_{\featuremat, \graph}(\node_i, \node_j)    
% \end{align}
% where the distance function is defined by the dot-product operation between feature representations in the final layer $\featuremat^{(K)}$. For the final clustering method (Line~\ref{alg:line:kmean} in Algorithm~\ref{algo:K-Medoids}), we choose to use K-Medoids instead of $k$K-Centr mainly due to two reasons: \\
% 1) Under similar assumptions as in Theorem~\ref{th:main}, we could see that K-Center is confined to a looser bound in terms of the total loss; that is:
% \begin{equation}
%\frac{1}{n}l(\algo_t|\graph,\featuremat,\labelvec)\leq c_0\max_i \min_{j\in \selected{0}} \|(S^KX)_i-(S^KX)_j\|_2 + \sqrt{\frac{\lossbound\log(1/\delta)}{2n}}
%  \frac{1}{n}\sum_{i=1}^n \min_{j\in \selected{0}}\|(S^KX)_i-(S^KX)_j\|_2\leq \. 
%\end{equation}

% \begin{theorem}
% \label{th:kcenter}
% Suppose the set $\selected{0}$ is a $\coversize$-cover of the nodes under the distance defined by $S^KX$, i.e.,  $\max_{i\in \nodeset}\min_{j\in \selected{0}}\|(S^KX)_i-(S^KX)_j\|_2\leq \delta$.
% Under the same assumptions and the same constant $c_0$ as in Theorem \ref{th:main}, with probability $1-\delta$ the expected inductive loss of $\algo_t$ satisfies
% \begin{equation}
%   \frac{1}{n}l(\algo_t|\graph,\featuremat,\labelvec)\leq c_0\coversize + \sqrt{\frac{\lossbound\log(1/\delta)}{2n}}   \label{eqn:bound_coreset}
% \end{equation}
% \end{theorem}
% The first term, proportional to the maximum of point-center distance, is larger than the mean point-center distance counter-part in K-Medoids. We visualize the difference in Figure~\ref{fig:vis}. \\
% 2) As K-Center is NP-Hard \citep{har2011geometric}, in order to get a more accurate solution, people use mixed integer programming (MIP) \citep{sener2017active} as the approximated algorithm, which can be much more time-consuming than K-Medoids based on Expectation Maximization (EM). An alternative solution is to use a greedy selection paradigm specified in Algorithm~\ref{algo:$k$-Cknter}. While being more efficient, the greedy algorithm will have inferior performances to MIP in applications such as image classifications with CNNs \citep{sener2017active}. We will elaborate more on these points in the Section~\ref{sec:exp_res}.

% \yw{pictures showing the difference of K-Medoids and K-Center}

% \yw{may delete the algorithm, its only a greedy-approximation}


%\begin{algorithm}[ht]
%	\caption{K-Center-Greedy%\yw{modify for }
%	}
%	\label{algo:$k$-Ck-center}
%	\begin{algorithmic}[1]        
%		\Require{Distance function $d_{\featuremat, \graph}(\cdot,\cdot)$, % $\featuremat^{(K)}$, 
%		existing pool $\selected{0}$ and a budget $b$}
%		\State Initialize $\selected{}=\selected{0}$\Comment{Warm start, $\selected{0}$ can be a small random selection}
%		\Repeat
%% 		\State $u=\arg\max_{i\in [\numtrain]\backslash \selected{}}\min_{j\in\selected{}}\Delta((\featuremat)^{(K)}_i,(\featuremat)^{(K)}_j)$
%		\State $u=\arg\max_{i\in [\numtrain]\backslash \selected{}}\min_{j\in\selected{}}d_{\featuremat, \graph}(\node_i,\node_j)$
%		\State $\selected{}=\selected{}\cup \{u\}$ 
%		\Until{$|\selected{}|=b+|\selected{0}|$}\\
%		\Return{$\selected{}$}
%	\end{algorithmic}
%\end{algorithm}

% \yw{tighter bound, illustrated in the experiment section}

% \yw{computation time, so in reality, people use $k$K-Center illustrated in the experiment section}



==> sections_iclr/conclusion.tex <==
\section{Conclusion}
We study the active learning problem in the node classification task for Graph Convolution Networks (GCNs). We propose a propagated node feature selection approach (FeatProp) to comply with the specific structure of GCNs and give a theoretical result characterizing the relation between its classification loss and the geometry of the propagated node features. Our empirical experiments also show that FeatProp outperforms the state-of-the-art AL methods consistently on most benchmark datasets. Note that FeatProp only focuses on sampling representative points in a meaningful (graph) representation, while uncertainty-based methods select the active nodes from a different criterion guided by labels, how to combine that category of methods with FeatProp in a principled way remains an open and yet interesting problem for us to explore.

==> sections_iclr/exp.tex <==
\section{Experiment}
%\subsection{Synthesized Experiment}
% \subsection{Experiment Details}

% \subsection{Dataset}
We evaluate the node classification performance of our selection method on the Cora, Citeseer, and PubMed network datasets \citep{yang2016revisiting}. We further supplement our experiment with an even denser network dataset CoraFull \citep{bojchevski2017deep} to illustrate the performance differences of the comparing approaches on a large-scale setting. Table~\ref{tab:dataset} summarizes the dataset statistics.

\begin{table}[ht]
    \centering
    \begin{tabular}{c|cccc}
        \toprule
        Data &\# Nodes &\# Edges &\# Classes & Feature size\\
        \midrule
        Cora & 2,708 &5,429 & 7 &3,703\\
        Citeseer & 3,327 &4,732 & 6 &1,433\\
        PubMed &19,717 &44,338 & 3 &500\\
       CoraFull &19,793 &126,842 &70 &8,710\\
        \bottomrule
    \end{tabular}
    \caption{Dataset statistics of different networks.}
    \label{tab:dataset}
\end{table}

\begin{table}[ht]
    \centering
    \begin{tabular}{c|cccc}
        \toprule
         & Cora & Citeseer &PubMed &CoraFull \\
        \midrule
        FeatProp & 239 & 622 & 1,506 &13,059\\
        CoresetMIP & 12,260 &13,257 & OOT &OOT\\
        Coreset-greedy & 44 & 46 & 509 & 636\\
        \bottomrule
    \end{tabular}
    \caption{Comparison of running time of 5 different runs in seconds between our algorithm (FeatProp) and Coreset. OOT denotes out-of-time. Note in order to get a more accurate solution, CoresetMIP costs much more time than Coreset-greedy.}
    \label{tab:time}
\end{table}

\begin{table}[ht] \centering \begin{tabular}{c|cccc} \toprule
 &Cora &Citeseer &PubMed &CoraFull\\
\midrule
Random &$59.83 \pm5.77$ &$48.79 \pm4.03$ &$71.66 \pm4.50$ &$10.75 \pm0.92$\\
Degree &$63.30 \pm0.55$ &$35.50 \pm0.82$ &$60.54 \pm0.38$ &$10.85 \pm0.30$\\
Uncertainty &$48.14 \pm8.18$ &$39.14 \pm4.52$ &$64.80 \pm8.21$ &$6.76 \pm0.72$\\
Coreset-greedy &$59.99 \pm4.59$ &$48.21 \pm3.78$ &$68.41 \pm4.50$ &$10.83 \pm1.28$\\
CoresetMIP &$55.86 \pm6.89$ &$46.76 \pm3.99$ &$-$ &$-$\\
AGE &$65.01 \pm2.43$ &$49.65 \pm5.19$ &$67.96 \pm2.73$ &$13.52 \pm0.81$\\
ANRMAB &$63.71 \pm4.34$ &$47.29 \pm3.33$ &$71.06 \pm4.82$ &$11.40 \pm0.98$\\
FeatProp &$\bm{74.89 \pm2.63}$ &$\bm{51.03 \pm2.80}$ &$\bm{73.20 \pm1.81}$ &$\bm{14.86 \pm0.70}$\\
\bottomrule \end{tabular} 
\caption{Comparison of Macro-F1$\pm$standard\_deviation averaged over different number of labeled nodes for training. Bold fonts represent the best methods. CorsetMIP does not scale up for PubMed and CoraFull datasets.}
\label{tab:macro-f1-gcn}
\end{table}

We evaluate the % \yx{inductive} 
Macro-F1 of the methods over the full set of nodes. The sizes of the budgets are fixed for all benchmark datasets. Specifically, we choose to select $10, 20, 40, 80$ and $160$ nodes as the budget sizes. After selecting the nodes, a two-layer GCN \footnote{In the past semi-supervised setting of citation networks, a two-layer GCN is the optimal structure for the node classification task \citep{kipf2016semi}. %the performances of GCNs are not sensitive to the number of layers. We choose this layer number as the result of both performance and efficiency considerations.
}, with $16$ hidden neurons, is trained as the prediction model. We use the Adam \citep{kingma2014adam} optimizer with a learning rate of $0.01$ and weight decay of $5\times 10^{-4}$. All the other hyperparameters are kept as in the default setting ($\beta_1=0.9,\beta_2=0.999$). To guarantee the convergence of the GCN, the model trained after $200$ epochs is used to evaluate the metric on the whole set. %\footnote{Note in this graph AL setting, we do not have a validation set.} %\yx{Is the best performance over 200 epochs chosen, or we evaluate at exactly 200 epochs?}
\subsection{Baselines}
\label{exp:comparing_methods}
We compared the following methods:
% We compared our AL strategy (FeatProp) with other representative strategies listed below: %\yx{I changed the wording a little bit}
% \yw{all the strategies share the same GCN structure after the selection of nodes}
\begin{itemize}
    % \item \yw{Baseline explanation}
    \item \textbf{Random:} Choosing the nodes uniformly from the whole vertex set.
    \item \textbf{Degree:} Choosing the nodes with the largest degrees. Note that this method does not consider the information of node features.
    % \item \textbf{FeatureClustering:} This method performs a K-Means clustering over the raw features. Nodes that have the closest representations to the centers are selected. This method does not consider the graph structure.
    \item \textbf{Uncertainty:} Similar to the methods in \cite{joshi2009multi}, we put the nodes with max-entropy % and max-margin (i.e. difference between best and second-best scores) 
    into the pool of instances. % \yw{whether to use a more accurate term.}
    \item \textbf{Coreset \citep{sener2017active}:} This method performs a K-Center clustering over the last hidden representations in the network. If time allows (on Cora and Citeseer), a robust mixture integer programming method as in \cite{sener2017active} (dubbed CoresetMIP) is adopted. We also apply a time-efficient approximation version (Coreset-greedy) % see Algorithm~\ref{algo:k-center}) 
    for all of the datasets. The center nodes are then selected into the pool. % In our experiments, we observe no explicit difference between CoresetMIP and Coreset-greedy.
    \item \textbf{AGE \citep{cai2017active}:} This method linearly combines three metrics -- graph centrality, information density, and uncertainty and select nodes with the highest scores.
    \item \textbf{ANRMAB \citep{gao2018active}:} This method enhances AGE by learning the combination weights of metrics through an exponential multi-arm-bandit updating rule.
    \item \textbf{FeatProp:} This is our method. We perform a K-Medoids clustering to the propogated features (Eqn. (\ref{eqn:dist})), where $X$ is the input node features. In the experiment, we adopts an efficient approximated K-Medoids algorithm which performs K-Means until convergence and select nodes cloesest to centers into the pool. 
    % Note that the distance function in our algorithm is based on (\ref{eqn:dist})
\end{itemize}

%\begin{figure}[htb]
%    \centering
%    \begin{subfigure}[b]{\textwidth}
%        \centering
%        \includegraphics[width=0.475\linewidth]{Cora.pdf}%
%        \hfill
%        \includegraphics[width=0.475\linewidth]{Citeseer.pdf}%
%    \end{subfigure}
%    \vskip\baselineskip
%    \begin{subfigure}[b]{\textwidth}
%        \centering
%        \includegraphics[width=0.475\linewidth]{PubMed.pdf}%
%        \hfill
%        \includegraphics[width=0.475\linewidth]{CoraFull.pdf}%
%    \end{subfigure}
%    \caption{Results of different approaches over benchmark datasets ( averaged from 5 different runs).}
%    \label{fig:main}
%\end{figure}

\begin{figure}[htb]
    \centering
    \includegraphics[width=0.82\linewidth]{All_macro.pdf}%
    \caption{Results of different approaches over benchmark datasets averaged from 5 different runs.}
\label{fig:main}
\end{figure}

\subsection{Experiment Results}
\label{sec:exp_res}
% We conducted experiments on active learning for all approaches. 
In our experiments, we start with a small set of nodes (5 nodes) sampled uniformly at random from the dataset as the initial pool. We run all experiments with 5 different random seeds and report the averaged classification accuracy as the metric. We plot the accuracy vs the number of labeled points. For approaches (Uncertainty, Coreset, AGE and ANRMAB) that require the current status/hidden representations from the classification model, a fully-trained model built from the previous budget pool is returned. For example, if the current budget is $40$, the model trained from $20$ examples selected by the same AL method is used. %\yw{We run the query algorithm iteratively; in other words, we solve the discrete optimization problem}

\textbf{Main results.} % \yw{update analysis with new baselines} 
As is shown in Figure~\ref{fig:main}, our method outperforms all the other baseline methods in most of the compared settings. It is noticeable that AGE and ANRMAB which use uncertainty score as their sub-component can achieve better performances than Uncertainty and are the second best methods in most of the cases. 
% Note that Coreset and Uncertainty focus on exactly different selection criteria -- either expressiveness of features or the current model confidence. We believe that the observation there is no clear clue for which method is superior is partially due to the fact that datasets of different characteristics favor distinct selection aspects.  % Furthermore, note that FeatureClustering cannot achieve even close performances as FeatProp in most of the datasets, which suggests that the raw features alone have quite different geometry distribution as the propagated ones. 
% It is noticeable that Random could achieve relatively good performances on small datasets (Cora and Citeseer). When the vertex size (PubMed and CoraFull) grows, which may require more insightful guidance from graphs and features, Random will no longer give out good scores. \yw{previous sentence not reliable}
% Moreover, it is interesting to find that in CoraFull with the densest linkage structure, Degree, which utilizes the graph information alone could produce a good result and is even better than other active learning baselines.  We believe that this is due to the fact that methods (Uncertainty/Coreset) requiring model statuses/hidden representations can be highly-unstable and are more likely to sample biased nodes with an overfitted model resulting from the small number of training points.
% the vast number of % as CoraFull has a total of $70$ different 
% classes, which is larger than most of the sample budgets.\yx{I feel it better not to emphasize \#nodes<\#classes here - this is kind of weird. Let's discuss}
% In this case, strong guidance from the graph structure helps more. Naturally, FeatProp with no dependence on GCN parameters will also be stable. 
We also show an averaged Macro-F1 with standard deviation across different number of labeled nodes in Table~\ref{tab:macro-f1-gcn}. It is interesting to find that our method has the second smallest standard deviation (Degree is deterministic in terms of node selection and the variance only comes from the training process) among all methods. We conjecture that this is due to the fact that other methods building upon uncertainty may suffer from highly variant model parameters at the beginning phase with very limited labeled nodes.

%\yw{noticeable that methods that neglect information such as Degree FeatureClustering usually have the worst performance among all methods} 

\textbf{Efficiency.} % \yw{comparison of time} 
We also compare the time expenses between our method and Coreset, which also involves a clustering sub-routine (K-Center), %Algorithm \ref{algo:k-center}) 
in Table~\ref{tab:time}. It is noticeable that in order to make Coreset more stable, CoresetMIP uses an extreme excess of time comparing to Coreset-greedy in the same setting.
% the extra large amount of time cost for the CoresetMIP version is unavoidable \yx{does unavoidable mean large here?} while the greedy algorithm takes much less time on the same setting. 
An interesting fact we could observe in Figure~\ref{fig:main} is that CoresetMIP and Coreset-greedy do not have too much performance difference on Citeseer, and Coreset-greedy is even better than CoresetMIP on Cora. This is quite different from the result in image classification tasks with CNNs \citep{sener2017active}. This phenomenon distinguishes the difference between graph node classification with traditional classification problems. We conjecture that this is partially due to the fact that the nodes no longer preserve independent embeddings after the GCN structure, which makes the original analysis of Coreset not applicable. %\yw{whehther this analysis is valid}

\begin{figure}[htb]
    \centering
    % \includegraphics[width=0.85\linewidth]{kcenter_kmeans.pdf}%
    \includegraphics[width=0.85\linewidth]{kcenter_kmeans_macro.pdf}%
    \caption{Results of different approaches over benchmark datasets averaged from 5 different runs. Similar to Coreset, the orange line denotes replacing the original distance function in Eqn. (\ref{eqn:dist}) with L2 distance from the final GCN layer. The blue line denotes the algorithm replacing the K-Medoids module with K-Center clustering.
    }
    \label{fig:kcenter_kmeans}
\end{figure}

%\begin{figure}[htb]
%    \centering
%    \includegraphics[width=0.85\linewidth]{kcenter_kmeans_kl.pdf}%
%    \caption{KL Divergence of the label of selected nodes vs true label distribution of different approaches over benchmark datasets aggregated from 5 different runs. FeatProp-kcenter denotes the algorithm replacing the K-Means module with K-Center clustering. The lower, the better.}
%    \label{fig:kcenter_kmeans_kl}
%\end{figure}
% \textbf{K-Center replacement.}
\textbf{Ablation study.}
It is crucial to select the proper distance function and clustering subroutine for FeatProp (Line~\ref{alg:line:dist} and Line~\ref{alg:line:kmean} in Algorithm~\ref{algo:K-Medoids}). As is discussed in Section~\ref{sec:not_coreset}, we test the differences with the variant of using the L2 distance from the final layer of GCN as the distance function and the one by setting K-Medoids choice with a K-Center replacement.
%It is possible to replace the K-Means clustering module in Algorithm ~\ref{algo:k-means} with the counter-part in Coreset (K-Center).
We compare these algorithms in Figure~\ref{fig:kcenter_kmeans}. As is demonstrated in the figure, the K-Center version (blue line) has a lower accuracy than the original FeatProp approach. This observation is compatible with our analysis in Section~\ref{sec:not_coreset} as K-Medoids comes with a tighter bound than K-Center in terms of the classification loss. Furthermore, as final layer representations are very sensitive to the small budget case, we observe that the network representation version (orange line) also generally shows a much deteriorated performance at the beginning stage. % We further investigate the sampled label distributions from these two methods and compute their KL-divergence with respect to the true label distribution in Figure~\ref{fig:kcenter_kmeans_kl}. We can perceive that FeatProp retrieves a more real-data-like sample set while FeatProp-kcenter is more biased, which we conjecture \yw{wording} is the main cause of its inferior performance.
%\yw{replace the clustering method with K-Center}

% \yw{comparison of label distribution, seems like that the distribution is not the closest to the true label distribution}
% \yw{here only put the comparison of label distributions related to FeatProp and FeatProp-kcenter}
% \yw{appendix of SGC, GCN comparison}

Though FeatProp is tailored for GCNs, we could also test the effectiveness of our algorithm over other GNN frameworks. Specifically, we compare the methods over a Simplified Graph Convolution (SGC)  \citep{wu2019simplifying} and obtain similar observations. Due to the space limit, we put the detailed results in the appendix.


==> sections_iclr/intro.tex <==
\section{Introduction}
Graph Neural Networks (GNN) \citep{kipf2016semi, velivckovic2017graph, hamilton2017inductive, wu2019simplifying} have been widely applied in many supervised and semi-supervised learning scenarios such as node classifications, edge predictions and graph classifications over the past few years. Though GNN frameworks are effective at fusing both the feature representations of nodes and the connectivity information, people are longing for enhancing the learning efficiency of such frameworks using limited annotated nodes.
% In the node classification task, which is the subject we center on, GNNs are shown to have good generalization ability via training with only dozens of annotated nodes. 
This property is in constant need as the budget for labeling is usually far less than the total number of nodes. 
For example, in biological problems where a graph represents the chemical structure \citep{gilmer2017neural, jin2018junction} of a certain drug assembled through atoms, it is not easy to obtain a detailed analysis of the function for each atom since getting expert labeling advice is very expensive. On the other hand, people can carefully design a small ``seeding pool'' so that by selecting ``representative'' nodes or atoms as the training set, a GNN can be trained to get an automatic estimation of the functions for all the remaining unlabeled ones.

Active Learning (AL) \citep{settles2009active,bodo2011active}, following this lead, provides solutions that select ``informative'' examples as the initial training set. 
While people have proposed various methods for active learning on graphs \citep{bilgic2010active,kuwadekar2011relational,moore2011active,rattigan2007exploiting}, active learning for GNN has received relatively few attention in this area. \cite{cai2017active} and \cite{gao2018active} are two major works that study active learning for GNN. 
The two papers both use three kinds of metrics to evaluate the training samples, namely uncertainty, information density, and graph centrality. The first two metrics make use of the GNN representations learnt using both node features and the graph; while they might be reasonable with a good (well-trained) GNN model, the metrics are not informative when the label budget is limited and/or the network weights are under-trained so that the learned representation is not good. On the other hand, graph centrality ignores the node features and might not get the real informative nodes. Further, methods proposed in \cite{cai2017active,gao2018active} only combine the scores using simple linear weighted-sum, which do not solve these problems principally.
% \yw{add a connecting sentence}
% These methods utilize previous active learning and graph metrics to indicate informativeness. Here, the active learning metrics only use the current network representation to compute scores and ignores the graph structure, whereas the graph metrics only use the graph connections and ignore the network representation. 
%Both methods use existing active learning metrics and graph centrality as informativeness scores, 
%and try to find a linear combination of scores to optimize performance. All these methods takes either the node representation or the raw graph structure into account; 
% None of these works have tried to combine the graph structure with node features.
% Active learning under the graph learning setting has received relatively few attention in this area, with the only two 
%\yw{should put in a more thorough literature} 
% The most common approach in AL is uncertainty sampling \citep{settles2009active} where the nodes that the current model is least certain about along with the training phase are selected. Another major stream of AL approaches is the clustering-based selection strategy. Coreset \citep{sener2017active}, as one representative method in this category, generates several anchor points so that each node's feature representation is within a close proximity to one of the anchors. Nodes that are closest to the anchors are selected as the representative initial training set.

% However, existing methods face yet new challenges when applied to the GNN setting\yw{citation}. Given the relatively small size of graphs, a GNN is prune to overfitting issues, and the uncalibrated predictions by a GNN usually do not represent the true informativeness of data points, which deteriorates the effectiveness of uncertainty-based methods. On the other hand, clustering-based approaches like Coreset do consider the relation of nodes through the graph, and therefore fail to identify the central nodes. 
% \yw{bridge the sentence between the prev part} In another aspect, however, being able to consider the GNN framework characteristics can potentially help select nodes that are not only representative of the data distribution but also to the training efficiency of the specific GNN structure.

We propose a method specifically designed for GNN that naturally avoids the problems of methods above\footnote{Our code will be released upon acceptance.}. Our method select the nodes based on node features propagated through the graph structure, making it less sensitive to inaccuracies of representation learnt by under-trained models. Then we cluster the nodes using K-Medoids clustering; K-Medoids is similar to the conventional K-Means, but constrains the centers to be real nodes in the graph.
% We give formal theoretical guarantees on the accuracy that our method can achieve, and conjecture that previous methods cannot achieve such bounds. 
% However, our experiments (see Figure~\ref{fig:main}) show that these existing methods perform similarly to random sampling in most cases when applied to the graph domain. We conjecture that this is because none of these methods expressly consider the downstream classification algorithms (i.e. GNN frameworks) which uses the graph structure to achieve a good performance. As traditional AL settings do not include such graphs, the selected samples therefore might not be representative enough when combined with GNN frameworks. %the same based on features or graphs.
% In this paper we propose a solution to GNN frameworks in the graph learning setting, to address this issue. %to avoid the aforementioned problems of existing methods.
% To the best of our knowledge, there is no previous AL work with the explicit consideration of GNN structures. % \yw{}
% However,
% all of the aforementioned methods are model-agnostic that view the back-end framework (i.e. classification algorithms) as blackboxes: uncertainty sampling only considers the final output while Coreset utilizes node feature representations from the second-to-last layer of the neural network. Performing any framework change will have no influence on these AL methods. In another aspect, however, different GNNs do differ in their structures, and being able to consider the structure characteristics can potentially help select nodes that are not only representative of the data distribution but also to the training efficiency of the specific GNN structure. To the best of our knowledge, there is no previous work that studies AL problems with the explicit model-aware consideration of GNN structures.
% In this work, we present, for the first time, a novel lightweight AL method  specifically designed for the Graph Convolution Network (GCN) \citep{kipf2016semi}, one of the most widely-used GNN structures. 
% Our method performs the node feature propagation succeeded by the K-Means clustering to select representative nodes %over propagated node features and choose the nodes most close to the centers as the training set, 
%  so that the information of the graph structure and the node features are fused in a similar way as the GNN does. 
Theoretical results and practical experiments prove the strength of our algorithm. 
%  We also compare our methods systematically with state-of-the-art AL methods. 
%  The contributions of our work are mainly three-fold: % \yw{}% \yw{rewording of the following contributions}:
\begin{itemize}
    % \item We propose a new AL method, tailored for GCNs, for the node classification task.
    \item We perform a theoretical analysis for our method and study the relation between its classification loss and the geometry of the propagated node features. 
    \item We show the advantage of our method over Coreset \citep{sener2017active} by comparing the bounds. We also conjecture that similar bounds are not achievable if we use raw unpropagated node features. 
    % We also conjecture that previous methods in active graph learning cannot achieve similar bounds.
    %superiority over one existing method -- Coreset 
    \item We compare our method with several AL methods and obtain the best performance over all benchmark datasets.
    % \yx{maybe some visualization?}
\end{itemize}



==> sections_iclr/related.tex <==
\section{Related Works}
% \yx{this section can be shorter and merged; let us decide later.}
% \yw{comparison between two existing AL on graph algorithms should be mentioned.}
% \subsection{Active Learning}
\textbf{Active Learning (AL)} aims at interactively choosing data points from the training pool to maximize model performances, and has been widely studied both in theory \citep{beygelzimer2008importance,hanneke2014theory} and practice \citep{settles2009active,Shen_2017}. Recently, \cite{sener2017active} proposes to compute a Coreset over the last-layer activation of a convolutional neural network. The method is designed for general-purpose neural networks, and does not take the graph structure into account.
%A central problem in AL is the tradeoff between exploration and exploitation: During exploration, we would like to select most representative training samples in the training set. This has resulted in clustering-based methods \citep{5670014,nguyen2004active,bodo2011active, DBLP:journals/jmlr/TsangKC05}. For exploitation, the algorithm aims to find the data point that results in the maximal information gain. Popular methods in this regime include model uncertainty \citep{yang2016active} and margin to the decision boundary \citep{DBLP:journals/jmlr/TongK01}. Recently there have been methods that try to combine exploitation and exploration. For example, Sener et al.\citep{sener2017active} computes a Coreset cover over the last-layer activations of a convolutional neural network. 
%However such methods are mostly model-agnostic which put no special attention for GNN structures that can potentially be helpful.
% meaning that changing the underlining structure of the neural network will do no influence on the AL procedures/hyperparameters.
%We discuss the relation between our method and Coreset in Section \ref{sec:not_coreset}. 

%Except for the AL method dealing with data on the normal Euclidean space, s
Early works on AL with graph-structured data \citep{DBLP:conf/colt/DasarathyNZ15,DBLP:conf/cvpr/AodhaCKB14} study non-parametric classification models with graph regularization. More recent works analyze active sampling under the graph signal processing framework \citep{GSP, Chen_graphSampling}. However, most of these works have focused on the denoising setting where the signal is smooth over the graphs and labels are noisy versions of node features. Similarly, optimal experimental design \citep{Expdesign_book,DBLP:journals/corr/abs-1711-05174} can also apply to graph data but primarily deals with linear regression problems, instead of nonlinear classification with discrete labels. %\yw{Move sentence to previous part}
%where it is shown that passive experimental design can leverage the graph structure well and active sampling does not buy further improvement over passive experimental design.  



% how to measure the ``informativeness'' of the unlabeled data. In general, people usually tackle this challenge from two aspects: either through prediction uncertainty of the current model to the data or through the data expressiveness along. 

% \begin{itemize}
%     \item \textbf{Uncertainty:} centers on 
%     \item \textbf{Data expressiveness:} Corset: The Coreset method centers on expressiveness; more on this in; many clustering methods belong to this category. Section~\ref{sec:not_coreset}. Considers CNN, but not GNN.

% \end{itemize}
% \subsection{Graph Neural Network}
\textbf{Graph Neural Networks (GNNs)}  \citep{hamilton2017inductive,velivckovic2017graph,kipf2016semi} are the emerging frameworks in the recent years when people try to model graph-structured data. Most of the GNN variants follow a multi-layer paradigm. In each layer, the network performs a message passing scheme, so that the feature representation of a node in the next layer could be some neighborhood aggregation from its previous layer. The final feature of a single node thus comprises of the information from a multi-hop neighborhood, and is usually universal and ``informative'' to be used for multiple tasks. % Noticeably, the layers could also be combined with pooling operations so that the network could output a single vectorized representation in the final layer which can be assumed to obtain a summary of the whole graph. Specifically, such GNN structures are shown empirically to achieve state-of-the-art performances in tasks including node classification, edge prediction and graph classifications.  
Recent works show the effectiveness of using GNNs in the AL setting. \cite{cai2017active}, for instance, proposes to linearly combine uncertainty, graph centrality and information density scores and obtains the optimal performance. \cite{gao2018active} further improves the result by using learnable combination of weights with multi-armed bandit techniques. Instead of combining different metrics, in this paper, we approach the problem by clustering propagated node features. We show that our one-step active design outperforms existing methods based on learnt network represenations, in the small label setting, while not degrading in performance for larger amounts of labeled data.
% Our work improves on these results by using propagated node features and K-Medoids clustering.
% As discussed above, 
% their metrics considers the network representation and graph structure separately,  while our metric can take both into account.
% cannot take information from features and graph structure into account jointly. 
% \yw{to be modified}
% However, nearly all of the works with GNNs proceed these problems in a supervised/semi-supervised way, while no active sampling is considered. 

% Although earlier works have studied active learning on graphs \citep{DBLP:conf/colt/DasarathyNZ15,DBLP:conf/cvpr/AodhaCKB14},
% To the best of our knowledge no previous works have studied AL with explicit consideration of GNN structures, which is one of the key contributions in our work.

% It is important to note that though cluster-based active learning has been studied in previous works \citep{nguyen2004active,bodo2011active}, there is no explicit model-aware consideration/analysis of any of the aforementioned approaches with GNN frameworks, which is one of the key contribution in our work.

